Combinatorial Bandits under Strategic Manipulations

Strategic behavior against sequential learning methods, such as "click framing" in real recommendation systems, have been widely observed. Motivated by such behavior we study the problem of combinatorial multi-armed bandits (CMAB) under strategic manipulations of rewards, where each arm can modify the emitted reward signals for its own interest. This characterization of the adversarial behavior is a relaxation of previously well-studied settings such as adversarial attacks and adversarial corruption. We propose a strategic variant of the combinatorial UCB algorithm, which has a regret of at most $O(m\log T + m B_{max})$ under strategic manipulations, where $T$ is the time horizon, $m$ is the number of arms, and $B_{max}$ is the maximum budget of an arm. We provide lower bounds on the budget for arms to incur certain regret of the bandit algorithm. Extensive experiments on online worker selection for crowdsourcing systems, online influence maximization and online recommendations with both synthetic and real datasets corroborate our theoretical findings on robustness and regret bounds, in a variety of regimes of manipulation budgets.

==> WSDM/algoproof.tex <==

We now propose a variant of combinatorial upper confidence bound algorithm that is robust to strategic manipulations of rewards in Algorithm \ref{algo}. The only mild assumption we maintain is that the learning algorithm has the knowledge of the largest budget possessed among all bandits arms, i.e, $B_{max}$. This is a relaxation of the assumptions made by \citet{pmlr-v119-feng20c} on strategic UCB algorithm, in which the learning algorithm has access to the cumulative use of budget at every time step. We start with a detailed description of the algorithm and then analyze the theoretical upper bound of regret, which enjoys $O(m \log{T} + m B_{max})$. 

For each arm $i$, our algorithm maintains a counter $K_{i,t-1}$ as the total number of times arm $i$ has been pulled up to time $t-1$ and $\widetilde{\mu}_{i,t} = \frac{\sum_{j=1}^{t-1} (x_{i,j}+ z_{i,j})}{K_{i,t-1}}$ as the empirical mean estimation based on the observations. At each time step, the algorithm computes the UCB estimation $\Bar{\mu}_{i,t}= \widetilde{\mu}_{i,t} + \sqrt{\frac{ 3 \log{t} }{2K_{i,t-1}}} + \frac{B_{max}}{K_{i,t-1}}$ for $i \in [m]$. With $\Bar{\mu}_{i,t}$, the $(\alpha, \beta)$-approximation oracle then outputs an approximately optimal arm subset $S_t \in \mathcal{S}$. The algorithm plays the return arm subset and update the counter $K_{i,t}$ and the estimation $\widetilde{\mu}_{i,t}$ accordingly. 

\begin{algorithm}[htb]
\DontPrintSemicolon
{\bf Input:}
Horizon $T$, number $m$ of arms, maximum budget $B_{max}$\;
{\bf Output:} Arm subset $S_t$\; 
  Initialize $K_{i,0} = 0$ and $\widetilde{\mu}_{i,0} = 0$ for $i \in [m]$\; 
  \For{t = 1 $\to$ m}{
    Play an arbitrary arm subset $S_t \in \mathcal{S}$ such that $t \in S_t$\; 
    $K_{i,t} = K_{i,t-1} + 1$ for $i \in S_t$\;
    $\widetilde{\mu}_j = x_{i,t}+z_{i,t}$ for $i \in S_t$ \;}
  \For{t = m+1 $\to$ T}{
  For $i \in [m]$, compute $\Bar{\mu}_{i,t}= \widetilde{\mu}_{i,t-1} + \sqrt{\frac{ 3 \log{t} }{2K_{i,t-1}}} + \frac{B_{max}}{K_{i,t-1}} $\;
  $S_t$ = {\textbf{oracle}}$(\Bar{\mu}_{1,t},\Bar{\mu}_{2,t},.....,\Bar{\mu}_{m,t})$\;
  Play arm subset $S_t$ and update 
  $K_{i,t} = K_{i,t-1} + 1$ and $ \widetilde{\mu}_{i,t} =  \frac{\sum_{j=1}^{t} (x_{i,j} + z_{i,j})}{K_{i,t}}$ for $i \in S_t$ \;
  }
\caption{SCUCB}
\label{algo}
\end{algorithm}

We first introduce a few notations that are used in our results. Define, for any arm $i\in[m]$, the suboptimality gaps as
\begin{align*}
        &\Delta^i_{min} = \alpha \cdot {OPT}_{\bm{\mu}} - \max\{r_{\bm{\mu}}(S) \mid S \in S_B, i \in S\}\,, \notag \\
     &\Delta^i_{max} = \alpha \cdot {OPT}_{\bm{\mu}} - \min\{r_{\bm{\mu}}(S) \mid S \in S_B, i \in S\}\,.
\end{align*}
We then denote the maximum and minimum of the suboptimality gaps as $\Delta_{max} = \max_{i \in [m]} \Delta^i_{max}\notag $ and $\Delta_{min} = \min_{i \in [m]} \Delta^i_{min}$.

The following lemma re-establish the canonical tail bound inequality in UCB under the setting of strategic manipulations. %The complete proof of Lemma \ref{lambda} is deferred to the appendix.
\begin{lemma}\label{lambda}
Let ${\Lambda}_{i,t} = \sqrt{\frac{3 \log{t} }{2K_{i,t-1}}} + \frac{\rho_{i,t-1}}{K_{i,t-1}}$, where $\rho_{i,t-1}$ is the total strategic budget spent by arm $i$ up to time $t-1$ and $K_{i,t-1}$ be the total number of pulls of arm $i$ up to time $t-1$. Define the event $E_t = \{ |\ \widetilde{\mu}_{i,t-1} - \mu_{i}| \leq \Lambda_{i,t}, \forall i \in [m]\}$, where $\mu_i$ is the true mean of arm $i$'s underlying distribution. 
Then, $\mathbb{P}(\lnot E_t)\leq 2m \cdot t^{-2}$.
\end{lemma}
\iffalse
\begin{proof}[Proof sketch] 
Denote $\hat{\mu}_{i,t-1} = \frac{\sum_{j=1}^{t-1} x_{i,j}}{K_{i,t-1}}$ as the estimation of the expected reward without the manipulated variable $z_{i,t}$. By the definition of $\hat{\mu}_{i,t}$ and $\widetilde{\mu}_{i,t}$,
\begin{align}
& \mathbb{P}\left(|\widetilde{\mu}_{i,t-1} - \mu_i| > \sqrt{\frac{3\log{t}}{2K_{i,t-1}}} + \frac{\rho_{i,t-1}}{K_{i,t-1}}\right) \notag \\
    %=\ & \mathbb{P}\left(\left|\hat{\mu}_{i,t-1} + \frac{\rho_{i,t-1}}{K_{i,t-1}}- \mu_i\right| > \sqrt{\frac{3\log{t}}{2K_{i,t-1}}} + \frac{\rho_{i,t-1}}{K_{i,t-1}} \ \right) \notag \\
    \leq\ & \mathbb{P}\left(\hat{\mu}_{i,t-1} - \mu_i > \sqrt{\frac{3\log{t}}{2K_{i,t-1}}} \ \right) + \mathbb{P}\left(\hat{\mu}_{i,t-1} - \mu_i <  -\sqrt{\frac{3\log{t}}{2K_{i,t-1}}}\right) \notag \\
    \leq\ & \sum_{s=1}^{t} \mathbb{P}\left(|\hat{\mu}_{i,{t-1}} - \mu_i|  > \sqrt{\frac{3\log{t}}{2s}}\ \right)\notag\\
    \leq\ & 2t\cdot \exp{(-3\log{t})} = \frac{2}{t^2} \,,\notag
\end{align}
where the last inequality follows the Chernoff-Hoeffding bound. By the union bound,
\[
\quad \mathbb{P}(\lnot E_t) = \mathbb{P}\left( \{ \forall i \in [m] ,\ |\widetilde{\mu}_{i,t-1} - \mu_{i}| > \Lambda_{i,t}\} \right)\leq 2m \cdot t^{-2} \,. \qedhere
\]
\end{proof}
\fi

Armed with Lemma \ref{lambda}, we present one of our main theorems, Theorem \ref{appendixA}, which gives the regret bound of $O(\log T)$ of SCUCB. The outline of the proof follows that of CUCB by \citet{pmlr-v28-chen13a}. To complete the proof, we carefully choose $\psi_t$, which controls the trade-off between the exploration and exploitation periods.% The full proof is deferred to the appendix.

\begin{theorem}
\label{appendixA}
The regret of the SCUCB algorithm with $m$ strategic arms in time horizon $T$ using an $(\alpha,\beta)$-approximation oracle is at most 
\begin{align}
 m\cdot\Delta_{max}\left( \frac{8B_{max} f^{-1}(\Delta_{min}) + 6\log{T}} {\left(f^{-1}(\Delta_{min})\right)^2} + \frac{\pi^2}{3}+1 \right)\,, \notag \nonumber
\end{align}
where $f^{-1}(\cdot)$ is the inverse bounded smoothness function.
\end{theorem}

\begin{proof}[Proof sketch]
We introduce a counter $N_i$ for each arm $i\in[m]$ after the $m$-round initialization and let $N_{i,t}$ be the value of $N_i$ at time $t$. We initialize $N_{i,m} = 1$. By definition, $\sum_{i \in [m]} N_{i,m} = m$. For $t > m$, the counter $N_{i,t}$ is updated as follows:
\begin{itemize}
    \item If $S_t \in S_B$, then $N_{{i'},t} = N_{{i'},t-1} + 1$ where $i' =$ $\argmin_{i \in S_t}$ $N_{i,t-1}$. In the case that $i'$ is not unique, we break ties arbitrarily;
    \item If $S_t \notin S_B$, then no counters will be updated. 
\end{itemize}  
As such, the total number of pulls of suboptimal arm subsets is less than or equal to $\sum_{i=1}^m N_{i,T}$.

Define $\psi_t = \frac{8B_{max}f^{-1}(\Delta_{min}) + 6\log{t}} {\left(f^{-1}(\Delta_{min})\right)^2} > c $, where $c$ is the larger solution of
\begin{align*}
\label{square}
    &(f^{-1}(\Delta_{min}))^2 c^2  + 16B_{max}^2 - ((8B_{max} f^{-1}(\Delta_{min})- 6\log{t}) c = 0 \,. %\notag
\end{align*}
%We use $\mathbb{I}\{\cdot\}$ to denote the indicator function, and $\mathbb{I}\{A\}$ is 1 if event $A$ is true and 0 otherwise. 
Then, we decompose the total number $\sum_{i=1}^m N_{i,T}$ of pulls of suboptimal arm subsets as
\begin{align}
\sum_{i=1}^m N_{i,T} = \ & m +\sum_{t=m+1}^T \mathbb{I}\{ S_t \in S_B\} \notag \\
=\ &m +\sum_{t=m+1}^T \sum_{i=1}^m \mathbb{I}\{ S_t \in S_B, N_{i,t} > N_{i,t-1}, N_{i,t-1} \leq \psi_t\} \notag \\
&+ \sum_{t=m+1}^T \sum_{i=1}^m \mathbb{I}\{ S_t \in S_B, N_{i,t} > N_{i,t-1}, N_{i,t-1} > \psi_t\}\notag \\
\leq \ & m + m\psi_T+\sum_{t=m+1}^T \mathbb{I}\{ S_t \in S_B,N_{i,t-1} > \psi_t, \forall i \in S_t\}\,. \notag
\end{align}

The inequality follows as $\sum_{t=m+1}^T \sum_{i=1}^m \mathbb{I}\{ S_t \in S_B, N_{i,t} > N_{i,t-1}, N_{i,t-1} \leq \psi_t\}$ can be trivially bounded by $m\psi_T$. Thus the key to bound the total number of pulls of suboptimal arm subset is to upper bound $\sum_{t=m+1}^T \mathbb{I}\{ S_t \in S_B,N_{i,t-1} > \psi_t, \forall i \in S_t\}$. Let $F_t$ denotes the event that the oracle fails to provide an $\alpha$-approximate arm subset with respect to the input vector $\Bar{\bm{\mu}} = (\Bar{\mu}_{1,t},\Bar{\mu}_{2,t},.....,\Bar{\mu}_{m,t})$. 
Then we can decompose $\sum_{t=m+1}^T \mathbb{I}\{ S_t \in S_B,N_{i,t-1} > \psi_t, \forall i \in S_t\}$ as 
\begin{align}
&\quad \sum_{t=m+1}^T \mathbb{I}\{ S_t \in S_B,N_{i,t-1} > \psi_t, \forall i \in S_t\}\notag\\
%&\leq \sum_{t=m+1}^T (\mathbb{I}\{F_t\} + \mathbb{I}\{ \lnot F_t, S_t \in S_B,N_{i,t-1} > \psi_t, \forall i \in S_t\})\notag\\
&\leq \sum_{t=m+1}^T (\mathbb{I}\{F_t\} + \mathbb{I}\{ \lnot F_t, S_t \in S_B,  K_{i,t-1} > \psi_t, \forall i \in S_t\})\notag \\
&\leq (T-m)(1-\beta) +  \mathbb{I}\{ \lnot F_t, S_t \in S_B, K_{i,t-1} > \psi_t, \forall i \in S_t\}\notag \,. \notag
\end{align}

By leveraging the monotonicity and smoothness assumptions of the reward function, we show that $\mathbb{P}(\{\lnot F_t, E_t,  S_t \in S_B, K_{i,t-1} > \psi_t, \forall i \in S_t\}) = 0$. Therefore, by the inclusion-exclusion principle,
\begin{align}
     \mathbb{P}(\{\lnot F_t, S_t \in S_B, K_{i,t-1} > \psi_t, \forall i \in S_t\}) 
     &\leq \mathbb{P}(\lnot E_t) \leq 2m \cdot t^{-2} \,.\notag
\end{align}
%where the last inequality comes from lemma \ref{lambda}. 

Leveraging the upper bound of total number of pulls of suboptimal arm subsets, the regret is bounded by
\begin{align}
    & \quad Regret_{\bm{\mu},\alpha,\beta}(T)
    \notag \\
    & \leq T\alpha \beta \cdot \text{OPT}_{\bm{\mu}} - \left( T\alpha\cdot \text{OPT}_{\bm{\mu}} - \mathbb{E} \left[ \sum_{i=1}^m N_{i,T} \right]\cdot \Delta_{max} \right)
    \notag \\
     &\leq m\cdot \Delta_{max}\left(\frac{8B_{max} f^{-1}(\Delta_{min}) + 6\log{T}} {\left(f^{-1}(\Delta_{min})\right)^2} + \frac{\pi^2}{3}+1\right)\,. \notag \qedhere
\end{align}
\end{proof}

It remains in question whether a bandit algorithm can achieve a regret upper bound sublinear in $B_{max}$. 
Our conjecture is negative.
In fact, under strategic manipulations of rewards, the design of robust bandit algorithms, e.g. UCB and $\epsilon$-greedy, is analogous to the design of outlier-robust mean estimation algorithms. Existing works on robust mean estimation, such as \citet{steinhardt_et_al:LIPIcs:2018:8368}, argue that, from an information theoretical point of view  mean estimation error must be depending on the variance of the data. Casting this argument to bandit with the strategic manipulation setting, we believe that a tight regret bound is unlikely to be independent of the strategic budget $B_{max}$. Moreover, Proposition 4 in \citet{steinhardt_et_al:LIPIcs:2018:8368} implies that the dependency on $B_{max}$ is linear. This corresponds to our linear dependency of regret in Theorem \ref{appendixA}.


==> WSDM/exp.tex <==
In this section, we evaluate our SCUCB algorithm empirically on synthetic data and three real applications, namely online worker selection in crowdsourcing, online recommendation, and online influence maximization.

\subsection{Baseline Algorithms}

We compare our proposed SCUCB algorithm with both stochastic and adversarial bandits algorithms that achieves optimal asymptotic regret in their settings.
\begin{enumerate}
    \item CUCB \cite{pmlr-v28-chen13a}. CUCB is the naive counterpart of our algorithm. The algorithm calculates a upper confidence interval for each arm and pick the best arm subset with the highest upper confidence interval. 
    \item TSCB \cite{wang2018thompson}. TSCB is the combinatorial version of the classical Thompson sampling algorithm. The algorithm maintain a prior beta distribution estimation for each arm and updates according to the received reward. At each time, the algorithm samples from the estimated distributions and pick actions according to the highest sample. 
    \item Combinatorial variant of EXP3 \cite{auer_nonstochastic_2002}. The algorithm maintains a weight for each arm and draw actions according to the normalized weight distribution. Upon receiving rewards, the algorithm update weight according to the classical EXP3 update rule. 
\end{enumerate}

\subsection{Synthetic Experiments}

We conduct experiments presented in this section with synthetic data and compare our proposed algorithm with its naive counter part. The approximation oracle is designed to succeed with probability $1$. Each bandit arm is modeled to follow a Bernoulli distribution with randomly populated $\mu \in [0,1]$ and all arms adapt LSI strategy. 
The arms in the optimal arm subset have a strategic budget of $0$ since additional strategic budget for optimal arms would only boost the performance of our algorithm. All other arms are equipped with a randomly allocated budget $B$,$ 0 \leq B \leq B_{max}$ by definition. 
As is typical in the bandit literature, for example in \citet{auer2002finite}, we evaluate both the naive and strategic CUCB algorithms on their tuned versions, where the UCB exploration parameter is scaled by a constant factor $\gamma \in [0,1]$. To ensure reproducible result, each experiment is repeated for $10$ random seeds and the averaged result is presented.  

\begin{table}[H]
\centering
\label{table:1}
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{5}{c}{Cumulative regret, Action size = 2, K = 10}                                       \\ \midrule
\multicolumn{1}{l|}{Dataset}        & \multicolumn{4}{c}{Synethetic}                                        \\ \midrule
\multicolumn{1}{l|}{Bmax}           & 70              & 90              & 110             & 130             \\
\multicolumn{1}{l|}{CUCB}           & 171.74          & 187.51          & 259.04          & 256.66          \\
\multicolumn{1}{l|}{\textbf{SCUCB}} & \textbf{143.85} & \textbf{172.57} & \textbf{208.53} & \textbf{233.57} \\ \bottomrule
\end{tabular}
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{5}{c}{Cumulative regret, Action size = 2, K = 20}                                        \\ \midrule
\multicolumn{1}{l|}{Dataset}        & \multicolumn{4}{c}{Synethetic}                                         \\ \midrule
\multicolumn{1}{l|}{Bmax}           & 70              & 90              & 110             & 130              \\
\multicolumn{1}{l|}{CUCB}           & 434.82          & 492.02          & 520.97          & 549.57           \\
\multicolumn{1}{l|}{\textbf{SCUCB}} & \textbf{301.57} & \textbf{365.94} & \textbf{450.10} & \textbf{505.453} \\ \bottomrule
\end{tabular}
\caption{Cumulative regret achieved by UCB and SCUCB with synthetic data with various action size.}
\end{table}

The first set of experiment is conducted with $K = \{10, 20\}$ arms through a time horizon of $T=5000$ time steps with maximum possible budget of $B_{max} = \{70, 90, 110, 130\}$. The algorithms are asked to select $\text{Action size} = 2$ arms as an arm subset at each time step. The cumulative regret incurred by CUCB and SCUCB algorithm are presented in the table \ref{table:1} where the performance of our proposed SCUCB algorithm is highlighted in bold text. Clearly, SCUCB demonstrated its effectiveness as it achieves significantly smaller regrets in various possible maximum strategic budget. 

The next two tables reveals the advantage of SCUCB algorithm with various size of action set. The experiments are conducted with time horizon of $T=5000$ time steps with $K = \{10, 20\}$ arms and maximum possible budget of $B_{max} = \{50\}$. The algorithms are asked to select $\text{Action size} = \{2, 4, 6, 8\}$ arms as an arm subset at each time step. Once again, our SCUCB outperforms its naive counterpart by achieving much smaller cumulative regret, for which numerical results are highlighted in bold text. 
\begin{table}[H]
\centering
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{5}{c}{Cumulative regret, Bmax = 50, K = 10}                                            \\ \midrule
\multicolumn{1}{l|}{Dataset}        & \multicolumn{4}{c}{Synethetic}                                       \\ \midrule
\multicolumn{1}{l|}{Action Size}    & 2               & 4               & 6               & 8              \\
\multicolumn{1}{l|}{CUCB}           & 140.21          & 150.88          & 158.22          & 123.91         \\
\multicolumn{1}{l|}{\textbf{SCUCB}} & \textbf{105.58} & \textbf{113.63} & \textbf{103.42} & \textbf{88.72} \\ \bottomrule
\end{tabular}
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{5}{c}{Cumulative regret, Bmax = 50, K = 20}                                             \\ \midrule
\multicolumn{1}{l|}{Dataset}        & \multicolumn{4}{c}{Synethetic}                                        \\ \midrule
\multicolumn{1}{l|}{Action Size}    & 2               & 4               & 6               & 8               \\
\multicolumn{1}{l|}{CUCB}           & 302.10          & 316.09          & 340.52          & 328.80          \\
\multicolumn{1}{l|}{\textbf{SCUCB}} & \textbf{232.23} & \textbf{247.32} & \textbf{268.27} & \textbf{306.77} \\ \bottomrule
\end{tabular}
\caption{Cumulative regret achieved by UCB and SCUCB with synthetic data with various $B_{max}$.}
\end{table}
%Synthetic, repeat = 10, T = 5000, arm = 10
To compare the two algorithms in details, we plot the cumulative regret incurred by algorithms against the time steps. It becomes apparent that the SCUCB algorithm features a cumulative regret versus time steps line that is much smaller than the one caused by CUCB even under a higher maximum possible strategic budget. We compare the two algorithm under settings where the maximize possible budget is $B_{max} = 70, 90$ and $B_{max} = 110, 130$.
\begin{figure}[H]
\centering
\subfigure[]{
\label{Fig1}
\includegraphics[width=3.8cm]{figs/B7090_K20_N10000.png}}
\subfigure[]{
\label{Fig2}
\includegraphics[width=3.8cm]{figs/B110130_K20_N10000.png}}
\caption{\ref{Fig1} Comparison of CUCB and SCUCB with $B_{max} = 70, 90$. \ref{Fig2} Comparison of CUCB and SCUCB with $B_{max} = 110, 130$.}
%\caption{\ref{Fig1} CUCB algorithm performance with maximize possible budget of $B_{max} = 70$ and SCUCB algorithm performance with maximize possible budget of $B_{max} = 70, 90$ \ref{Fig2} C CUCB algorithm performance with maximize possible budget of $B_{max} = 110$ and SCUCB algorithm performance with maximize possible budget of $B_{max} = 110, 130$.}
\end{figure}

\subsection{Online Worker Selection in Crowdsourcing Systems}
We simulated a online crowdsourcing system that has a workflow resembled by \ref{crowdsys} and model it as a combinatorial bandits problem. We performed extensive empirical analysis of our SCUCB algorithm against CUCB, the combinatorial version of Thompson sampling and EXP3. The experiments were conducted with the Amazon sentiment dataset, where Amazon items reviews are labeled 'is/is not book' or 'is/is not negative \cite{Krivosheev:2018:CCM:3290265.3274366}. We split the dataset into two, where 'is book' contains data that only has labels 'is/is not book' and 'is negative' contains data that only has labels 'is/is not negative'. Both dataset consists of 7803 reviews, 284 workers, and 1011 tasks. 
The correctness of workers and tasks can be visualized by the figures as below. 
\begin{figure}[H]
\centering
\subfigure[]{
\label{worker}
\includegraphics[width=3.8cm]{figs/worker_visual.png}}
\subfigure[]{
\label{task}
\includegraphics[scale = 0.28]{figs/task_visual.png}}
\caption{\ref{worker} Visualization of correctness of worker's labels. \ref{task}Visualization of correctness of task's labels.}
\end{figure}

For each task, the data contains responses from 5 workers and the crowdsourcing platform is asked to select 2, 3, or 4 workers at each time step. To measure the performance of the algorithms, we made the assumption that the reward is monotonically correlated to the accuracy of label compared to ground truth label. Thus, we define the reward to be 1, if the worker's label is the same with ground truth label and 0 otherwise. To model the strategic behavior of the workers, we model each worker with a randomly allocated strategic level $s \in [0,1]$ such that the worker provides its honest response with probability $s$. 

\begin{table}[H]
\label{first}
\centering
\begin{tabular}{@{}lccc@{}}
\toprule
\multicolumn{4}{c}{Crowdsourcing (Cumulative Reward), Bmax = 500}                            \\ \midrule
\multicolumn{1}{l|}{Dataset}        & \multicolumn{3}{c}{is\_book}                           \\ \midrule
\multicolumn{1}{l|}{Action size}    & 2                & 3                & 4                \\ \midrule
\multicolumn{1}{l|}{CUCB}           & 31672.6          & 46181.2          & 68244.6          \\
\multicolumn{1}{l|}{TSCB}          & 19853.0          & 34226.2          & 60621.2          \\
\multicolumn{1}{l|}{EXP3}           & 31569.6          & 46570.6          & 68482.2          \\
\multicolumn{1}{l|}{\textbf{SCUCB}} & \textbf{32082.6} & \textbf{46623.6} & \textbf{68524.6} \\ \bottomrule
\end{tabular}
\begin{tabular}{@{}lccc@{}}
\toprule
\multicolumn{4}{c}{Crowdsourcing (Cumulative Regret), Bmax = 500}                            \\ \midrule
\multicolumn{1}{l|}{Dataset}        & \multicolumn{3}{c}{is\_book}                           \\ \midrule
\multicolumn{1}{l|}{Action size}    & 2                & 3                & 4                \\ \midrule
\multicolumn{1}{l|}{CUCB}           & 27787.4          & 42198.8          & 48125.4          \\
\multicolumn{1}{l|}{TSCB}          & 39607.0          & 54153.8          & 55748.8          \\
\multicolumn{1}{l|}{EXP3}           & 27890.4          & 41809.4          & 47887.8          \\
\multicolumn{1}{l|}{\textbf{SCUCB}} & \textbf{27377.4} & \textbf{41756.4} & \textbf{47845.4} \\ \bottomrule
\end{tabular}
\end{table}
\begin{table}[H]\centering
\begin{tabular}{@{}lccc@{}}
\toprule
\multicolumn{4}{c}{Crowdsourcing (Cumulative Reward), Bmax = 500}                            \\ \midrule
\multicolumn{1}{l|}{Dataset}        & \multicolumn{3}{c}{is\_negative}                       \\ \midrule
\multicolumn{1}{l|}{Action size}    & 2                & 3                & 4                \\ \midrule
\multicolumn{1}{l|}{CUCB}           & 31108.8          & 44757.6          & 59424.8          \\
\multicolumn{1}{l|}{TSCB}          & 17240.6          & 32010.4          & 51109.0          \\
\multicolumn{1}{l|}{EXP3}           & 30879.0          & 44767.2          & 58207.8          \\
\multicolumn{1}{l|}{\textbf{SCUCB}} & \textbf{31759.0} & \textbf{44843.4} & \textbf{59441.4} \\ \bottomrule
\end{tabular}
\begin{tabular}{@{}lccc@{}}
\toprule
\multicolumn{4}{c}{Crowdsourcing (Cumulative Regret), Bmax = 500}                            \\ \midrule
\multicolumn{1}{l|}{Dataset}        & \multicolumn{3}{c}{is\_negative}                       \\ \midrule
\multicolumn{1}{l|}{Action size}    & 2                & 3                & 4                \\ \midrule
\multicolumn{1}{l|}{CUCB}           & 28411.2          & 43566.2          & 56465.2          \\
\multicolumn{1}{l|}{TSCB}          & 42279.4          & 56279.6          & 64781.0          \\
\multicolumn{1}{l|}{EXP3}           & 28641.0          & 43523.4          & 57682.2          \\
\multicolumn{1}{l|}{\textbf{SCUCB}} & \textbf{27761.0} & \textbf{43446.6} & \textbf{56448.6} \\ \bottomrule
\end{tabular}

\caption{Cumulative rewards and cumulative regret attained by SCUCB and baseline algorithms with various action size on isbook dataset and isnegative datase.}
\end{table}
For the first set of experiments, we choose the maximum possible strategic budget to be $B_{max} = 500$. For actions size of $2, 3, 4$. We obtain the following cumulative rewards and cumulative regret results where SCUCB's performance is highlight in bold text. To ensure reproducible results, each experiment is repeated for 5 times and the averaged result is presented. 

To further investigate the effect of maximum possible strategic budget on the performance of algorithms, we fix the size of action size to be 2 and plot the cumulative reward/cumulative regret incurred by each algorithm again $B_{max} \in [100, 700]$. Regardless of the $B_{max}$ value, our proposed SCUCB algorithm consistently outperforms other methods. For better visualization, we omit the line for combinatorial Thompson sampling due to its relatively weaker performance. 
\begin{figure}[H]
\centering
\subfigure[]{
\label{culre}
\includegraphics[width=3.8cm]{figs/culre.png}}
\subfigure[]{
\label{culreg}
\includegraphics[width=3.8cm]{figs/reg.png}}
\caption{\ref{culre} Cumulative rewards attained by algorithms with various level of $B_{max}$.  \ref{culreg} Cumulative regrets attained by algorithms with various level of $B_{max}$.  }
\end{figure}

The results of our crowdsourcing experiments reveals the robustness of our SCUCB algorithm under strategic manipulations. It also indicates the performance of adversarial and stochastic bandits algorithms under strategic manipulations. The combinatorial variant of Thompson sampling is vulnerable under manipulations, which agrees with our expectation given that the algorithm is a Bayesian algorithm in nature and is heavily relying on estimating the underlying distribution of arms. Its estimation can be easily perturbed under strategic manipulation, and thus leads to undesired performance results. It is also expected that the SCUCB algorithm far outperform its naive counterpart, CUCB algorithm. The combinatorial version of EXP3 algorithm is the most competitive algorithm with our SCUCB. As the EXP3 algorithm was originally designed for pure adversarial setting, the algorithm has some robustness under strategic manipulations. Shown in the Figure \ref{culrereg}, the combinatorial EXP3 algorithm consistently show robustness across various level of maximum possible strategic budget. However, as our SCUCB algorithm considers the maximum possible strategic budget and thus more adaptive, SCUCB far outperforms EXP3CB as $B_{max}$ increases. 

\subsection{Online Recommendation System}

Online recommendation is a classic example of combinatorial bandits in applications. We evaluated algorithms in the latest MovieLens dataset which contains 9742 movies and 100837 rating of the movies with each rating being $1 - 5$ \cite{10.1145/2827872}. We compare the algorithms based on the total values of ratings received, i.e. recommending a movie and receiving a rating of 5 is more desired than recommending a movie and receiving a rating of 1. 
\begin{figure}[H]
\centering
\includegraphics[width=7cm]{figs/arch.png}
\caption{Experiment set up of online recommendation.}
\end{figure}
As the dataset may consists of unbalanced data for each movie, we adapted collaborative filtering and $k$-means clustering into our evaluation system. We used the collaborative filtered for training and testing and instead of recommending movies, we clustered the movies by $k$-means clustering and asked bandits algorithm to choose one cluster at each time. The movie with the highest rating in the chosen cluster is recommended. The workflow of the experiment set up is summarized in above diagram. 

We performed the evaluation with various number of clusters (10, 20 or 30) and $B_{max} = 30, 50, 70$ through a time horizon of $T = 500$. The results presented below are averages over 5 runs to ensure reproducibility. From the tables below, we concludes the effectiveness of SCUCB algorithm, which performance is highlighted in bold text. 
\begin{table}[H]
\centering
\begin{tabular}{@{}lccc@{}}
\toprule
\multicolumn{4}{c}{Recsys (Cumulative Reward), T=500, 10 clusters}                          \\ \midrule
\multicolumn{1}{l|}{Dataset}       & \multicolumn{3}{c}{Movielens}                          \\ \midrule
\multicolumn{1}{l|}{Bmax}          & 30               & 50               & 70               \\ \midrule
\multicolumn{1}{l|}{UCB}           & 2297.60          & 2494.36          & 2631.02          \\
\multicolumn{1}{l|}{TS}            & 2160.14          & 2314.76          & 2468.26          \\
\multicolumn{1}{l|}{EXP3}          & 2181.11          & 2449.28          & 2430.96          \\
\multicolumn{1}{l|}{\textbf{SUCB}} & \textbf{2305.75} & \textbf{2314.76} & \textbf{2636.07} \\ \bottomrule
\end{tabular}
\begin{tabular}{@{}lccc@{}}
\toprule
\multicolumn{4}{c}{Recsys (Cumulative Reward), T=500, 20 clusters}                          \\ \midrule
\multicolumn{1}{l|}{Dataset}       & \multicolumn{3}{c}{Movielens}                          \\ \midrule
\multicolumn{1}{l|}{Bmax}          & 30               & 50               & 70               \\ \midrule
\multicolumn{1}{l|}{UCB}           & 2469.93          & 2336.92          & 2159.25          \\
\multicolumn{1}{l|}{TS}            & 2260.20          & 1850.55          & 1905.42          \\
\multicolumn{1}{l|}{EXP3}          & 2380.74          & 2317.82          & 2025.39          \\
\multicolumn{1}{l|}{\textbf{SUCB}} & \textbf{2474.69} & \textbf{2341.19} & \textbf{2177.70} \\ \bottomrule
\end{tabular}
\begin{tabular}{@{}lccc@{}}
\toprule
\multicolumn{4}{c}{Recsys (Cumulative Reward), T=500, 30 clusters}                                       \\ \midrule
\multicolumn{1}{l|}{Dataset}       & \multicolumn{3}{c}{Movielens}                          \\ \midrule
\multicolumn{1}{l|}{Bmax}          & 30               & 50               & 70               \\\midrule
\multicolumn{1}{l|}{UCB}           & 2443.57          & 2393.88          & 2472.31          \\
\multicolumn{1}{l|}{TS}            & 2132.16          & 2248.56          & 1855.14          \\
\multicolumn{1}{l|}{EXP3}          & 2368.42          & 2265.32          & 2339.49          \\
\multicolumn{1}{l|}{\textbf{SUCB}} & \textbf{2436.43} & \textbf{2397.72} & \textbf{2476.52} \\ \bottomrule
\end{tabular}
\caption{Cumulative rewards attained by algorithms with different number of clusters $10, 20, 30$ and different level of $\{B_{max} = 30, 50, 70\}$ across 500 time steps. }
\end{table}

\subsection{Online Influence Maximization}

We implemented the online influence maximization with an offline influence maximization algorithm TIM as our oracle \cite{10.1145/2588555.2593670}. TIM is one of the offline influence maximization algorithm that achieves asymptotic optimality. We perform the experiments on two datasets. One is a simulation dataset with 16 nodes and 44 edges, the other is a 100 nodes subset from Digg dataset, where each nodes represents a user from Digg website \cite{nr}. We simulate the connectivity of edges at each time step by randomly assigning each edge a connectivity probability at the start of the experiment. 

\begin{figure}[hbt!]
\centering
\subfigure[]{
\label{test_graph}
\includegraphics[width=3.6cm]{figs/test_graph.png}}
\subfigure[]{
\label{16c2}
\includegraphics[width=3.6cm]{figs/test.png}}
\caption{\ref{test_graph} Visualization of synthetic graph for evaluation. \ref{16c2} Mean rewards attained by algorithms.}
\end{figure}

Figure \ref{test_graph} visualizes the synthetic graph we created for evaluation. We then tested the algorithms over $T = 800$ time steps with action size of 2 and maximum possible strategic budget of $B_{max} = 300$. Figure \ref{16c2} show the effectiveness of algorithms by evaluating based on the averaged nodes influenced. To ensure reproducible results, we calculate the mean of nodes influence over 100 trials. For better visualization, we kept a running mean over 50 time steps to smooth the lines. 

We then investigate the effect of action size and the results are summarized in the following two tables.
\begin{table}[hbt!]
\centering
\begin{tabular}{@{}ccccc@{}}
\toprule
\multicolumn{5}{c}{OIM (Averaged Final Reward), Bmax = 200}                                   \\ \midrule
\multicolumn{1}{l|}{Dataset}        & \multicolumn{3}{c}{Synthetic, 16 nodes, 44 edges}         \\ \midrule
\multicolumn{1}{l|}{Action size}       & 2      & 4      & 6       & 8       \\ \midrule
\multicolumn{1}{c|}{CUCB}   & 5.46          & 6.54          & 10.4           & 12.5           \\
\multicolumn{1}{c|}{TSCB}  & 6.7           & 8.50           & 10.44          & 12.7           \\
\multicolumn{1}{c|}{EXP3CB} & 5.86          & 8.14          & 10.34          & 12.46          \\
\multicolumn{1}{c|}{\textbf{SCUCB}}  & \textbf{7.44} & \textbf{9.32} & \textbf{11.16} & \textbf{13.04} \\ \bottomrule
\end{tabular}
\begin{tabular}{@{}lccc@{}}
\toprule
\multicolumn{4}{c}{OIM (Averaged Final Reward), Bmax = 200}                       \\ \midrule
\multicolumn{1}{l|}{Dataset}        & \multicolumn{3}{c}{digg, 100 nodes}         \\ \midrule
\multicolumn{1}{l|}{Action size}    & 10             & 15             & 20        \\ \midrule
\multicolumn{1}{l|}{CUCB}           & 15.64          & 20.64          & 25.32           \\
\multicolumn{1}{l|}{TSCB}          & 16.30          & 21.62          & 26.08          \\
\multicolumn{1}{l|}{EXP3}           & 12.16          & 17.76          & 21.72          \\
\multicolumn{1}{l|}{\textbf{SCUCB}} & \textbf{16.56} & \textbf{22.16} & \textbf{26.14} \\ \bottomrule
\end{tabular}
\caption{Averaged final rewards attained by algorithms with synthetic and Digg dataset with action size of 2, 800 time steps and $B_{max} = 200$.}
\end{table}



\iffalse
\paragraph{Experiment setting} 

We conduct the experiments with 10 arms where each arm subset constitutes $2$ arms unless otherwise specified. The time horizon is set to be $T = 5\times 10^3$ and the approximation oracle is designed to succeed with probability $1$. Each bandit arm follows a Bernoulli distribution with randomly populated $\mu \in [0,1]$ and all arms adapt LSI except in the discussion of arm strategies. 
The arms in the optimal arm subset have a strategic budget of $0$ and all other arms are equipped with the same strategic budget, which is $B_{max}$ by definition. The setting of heterogeneous budgets is discussed in the appendix. 
As is typical in the bandit literature, for example in \citet{auer2002finite}, we evaluate both naive and strategic CUCB algorithms on their tuned versions, where the UCB exploration parameter is scaled by a constant factor $\gamma \in [0,1]$. Each experiment is repeated $10$ times and the averaged result is presented. 

\begin{figure*}[htbp]
\centering
\subfigure[]{
\label{Fig1}
\includegraphics[scale=0.3]{figs/diff_B.png}}
\subfigure[]{
\label{Fig2}
\includegraphics[scale=0.24]{figs/linearB.png}}
\subfigure[]{
\label{Fig3}
\includegraphics[scale=0.3]{figs/LSI2.png}}
\subfigure[]{
\label{Fig4}
\includegraphics[scale=0.3]{figs/50arm.png}}

\caption{\ref{Fig1} Cumulative regret v.s. time horizon under different maximum budgets; \ref{Fig2} Cumulative regret v.s. strategic budget; \ref{Fig3} Cumulative regret under the LSI strategy and random strategy; \ref{Fig4} Cumulative regret v.s. time horizon under different number of arms in each arm subset ($B_{max} = 50$).}
\end{figure*}
%Effect of tuning UCB confidence parameter
\paragraph{Cumulative regret v.s. maximum budgets} We experiment with $B_{max} \in \{0, 10, 50, 100\}$ and $\gamma = 0.2$. Figure \ref{Fig1} highlights the failure of naive CUCB as the regret grows linearly with respect to $T$. In comparison, the regret grows in a logarithmic fashion with strategic CUCB, which agrees with our theoretical finding of the $O(\log T)$ regret bound. 
%This confirms our regret analysis result in Theorem \ref{appendixA}.

\paragraph{Cumulative regret v.s strategic budget} We conduct our empirical study with and the strategic budget ranging from $1$ to $100$ under $\gamma = 0.2$. Figure \ref{Fig2} shows that the regret is linear with the largest strategic budget $B_{max}$ under both strategic CUCB and naive CUCB, which agrees with our linear term on the budget in Theorem \ref{appendixA}. 
%This attests to our theoretical bound of regret being $O(B_{max})$ under strategic CUCB. 
We observe that, though at a small value of $B_{max}$ CUCB display unstable performance, strategic CUCB can achieve much lower regret than that of naive CUCB in general. We, therefore, conclude the superiority of strategic CUCB in small-budget and large-budget regimes.

\paragraph{Cumulative regret under LSI strategy and random strategy} We simulate the random strategy for arms as arms randomly spend a budget that is generated from a standard uniform distribution in each round. 
%We stimulate the random strategy for arms, where the arms randomly spend part of its strategic budget in probability, simulated by uniform random seed, each time the arm is pulled. 
It is illustrated in Figure \ref{Fig3} that regardless of the choice of the bandit learning algorithm, the regret under LSI is higher than the regret under a random strategy. As is discussed previously, LSI strategy is one of the most powerful strategies that strategic arms can perform to hamper regret. The effect of strategies with collusion is demonstrated in the appendix. 

\paragraph{Cumulative regret v.s. different arm subset size} We relax the number of arms in each arm subset from $2$ to $4$ and $6$ to observe the sensitivity with respect to this parameter. We choose naive CUCB with $4$ arms in each arm subset as a baseline and the maximum budget is set to be $50$. As shown in Figure \ref{Fig4}, our algorithm outperforms naive CUCB regardless of the number of arms in each arm subset, which indicates the robustness of strategic CUCB on the arm subset size.

\fi

==> WSDM/formulation.tex <==
We consider the problem of combinatorial multi-armed bandits (CMAB) under the setting of strategic arms. In strategic CMAB, each arm is given a budget and the arm can strategically increase its emitted reward signals cumulatively up to this budget \emph{for its own interest}. This problem is a Stackelberg game which involves two parties. The bandit learning algorithm is deployed first to maximize its cumulative reward under the best response of the followers. The $m$ strategic bandits arms then deplete their budget where each of them aims to maximize its expected number of pulls. Knowing the principal's strategy and other followers' budget information, the followers are assumed to place their strategies according to the dominant Nash equilibrium between them. 

Formally, given a time horizon $T$, the the bandit learning algorithm is asked to pull a subset of arms, denoted by an arm subset $S_t \in \mathcal{S} $ at each time $t\in [T]$, where $\mathcal{S} = { \{0,1\}^{m}} $ is the set of all possible arm subsets. At time $t$, based on the principal's choice of arm subset, stochastic rewards $x_{i,t}$ are generated by arm $i$ from the underlying $1$-sub-Gaussian distribution with mean $\mu_i$, independent of other arms in $S_t$. The principal does not observe these rewards. Instead, each arm can increase the emitted reward signal by an arbitrary amount $z_{i,t}\ge 0$, as long as the cumulative manipulation over the horizon does not exceed a given budget $B_i$. The principal then receives the semi-bandit feedback $\{x_{i,t}+z_{i,t}\}_{i\in S_t}$.

%The reward of playing arm subset $S$ at time $t$ is decided by a stochastic reward function $R_t(S)$, which is a function of $\{x_{i,t}\}_{i\in S}$. 
Let $\bm{\mu} = (\mu_1, \mu_2, ..., \mu_i) $ be the vector of expectations of all arms. The expected reward of playing any arm subset S in
any round $r_{\bm{\mu}}(S) = \mathbb{E}[R_t(S)]$,which is a function of arm subset $S$ and $\bm{\mu}$. The reward function $r_{\bm{\mu}}(S)$ is assumed to satisfy two axioms:
\begin{itemize}
    \item \textbf{Monotonicity.} The expected reward of playing any arm subset $S \in \mathcal{S}$ is monotonically non-decreasing with respect to the expected reward vector. That is, if for all $i \in [m], \mu_i \leq \mu_{i}'$, then $r_{\bm{\mu}}(S) \leq r_{\bm{\mu}'}(S)$.
    \item \textbf{Bounded smoothness.} There exists a strictly increasing function $f(\cdot)$, termed the bounded smoothness function, such that for any two expected reward vectors $\bm{\mu}$ and $\bm{\mu'}$ satisfying $\|\bm{\mu}-\bm{\mu'}\|_{\infty}\le \Lambda $, we have $|r_{\bm{\mu}} - r_{\bm{\mu'}}| \leq f({\Lambda})$.
\end{itemize}
These axioms cover a rich set of reward functions and the explicit forms of $R_t(S)$ and $r_{\bm{\mu}}(S)$ are not needed to be specified \citep{pmlr-v28-chen13a}.

Without loss of generality, assume that $S^\ast = \argmax_{S\subseteq \mathcal{S}} r_{\bm{\mu}}(S)$ is the unique optimal subset of arms. When placing reward manipulations, each strategic arm has access to its own history $h_{i,t} = \{I_{i,t'}, x_{i,t'}, z_{i,t'}\}_{t'\ge 1}$, where $I_{i,t'}$ is the indicator of whether arm $i$ is pulled at time $t'$ and $t' < t$. The strategy of arm $i$ is determined by a function that maps this history to a manipulation $z_{i,t}$, as $Z_{i,t} \colon h_{i,t-1} \to \mathbb{R}$. Without loss of generality, we assume that arms in the optimal arm subset $i\in S^\ast$ have strategic budgets of $0$, which restricts their $z_{i,t}$ to be $0$.

In the combinatorial setting, even with the exact reward vector $\bm\mu$ provided, it can be hard to exactly compute the optimized $r_{\bm{\mu}}(S)$. In view of this, many have studied probabilistic approximation algorithms in combinatorial problems, which indicates that an ($\alpha,\beta$)-approximation oracle defined below can be usually available. 

\begin{definition}[Approximation oracle]
Let $0\le \alpha,\beta \leq 1$ and define ${OPT}_{\bm{\mu}} = \max_{S\in \mathcal{S}} r_{\bm{\mu}}(S)$. 
An oracle is called an ($\alpha,\beta$)-approximation oracle if it takes an expected reward vector $\bm{\mu}$ as input and outputs an arm subset $S \in \mathcal{S}$ such that $\mathbb{P}(r_{\bm{\mu}}(S) \geq \alpha \cdot {OPT}_{\bm{\mu}}) \geq \beta$. That is, the oracle gives an arm subset $S$ that is at least as good as $\alpha$ times the reward of an optimal arm subset with probability at least $\beta$. 
\end{definition}
Denote ${S_B} = \{ r_{\bm{\mu}}(S) < \alpha \cdot {OPT}_{\bm{\mu}} | S \in \mathcal{S}\}$ to be the set of suboptimal arm subsets under the approximation oracle. 
Note that a suboptimal arm subset can be given by the oracle for two reasons. The ($\alpha,\beta$)-approximation oracle can fail, which happens with probability at most $1-\beta$. The estimation of $\bm{\mu}$ can deviate from the true value by a significant amount, resulting in accurate input to the oracle.

The objective of the principal is to maximize the expected cumulative reward before manipulation over the time horizon $T$. Equivalently, the principal minimizes the regret, the cumulative difference between the scaled optimal reward and expected actual reward, as defined below. 

\begin{definition}[Regret]
With access to an ($\alpha,\beta$)-\textit{approximation oracle}, the regret of a combinatorial bandit algorithm for $T$ rounds is
\[
Regret_{\bm{\mu},\alpha,\beta}(T) = T \cdot \alpha \cdot \beta \cdot {OPT}_{\bm{\mu}} - \mathbb{E}\big[\sum^T_{t=1}r_{\bm{\mu}}(S_t)\big]\,,
\]
where the randomness in $\mathbb{E}[\sum^T_{t=1}r_{\bm{\mu}}(S_t)]$ involves the stochasticity of the bandit algorithm and the oracle.
\end{definition}

The objective of each strategic arm $i\in [m]\setminus S^{\ast}$, however, is to maximize the number $\sum_{t=1}^T I_{i,t}$ of times it is pulled over the time horizon. To achieve this, the arm needs to confuse the principal by deviating the emitted reward signals up to the possessed budget. % For a fixed bandit algorithm of the principal, the budget deployment strategies of the arms are assumed to follow the dominant Nash equilibrium $NE$. With the principal, this Stackelberg game writes
\iffalse
\begin{equation*}
\begin{aligned}
& \underset{S_t}{\mathrm{maximize}}
& & Regret_{\bm{\mu},\alpha,\beta}(T) \\
& \mathrm{subject}\text{ }\mathrm{to}
& & z_{i,t} = \argmax_{NE} \sum_{t=1}^T I_{i,t}, \ \text{for}\ t\in [T],\ i\in [m]\setminus S^*\,, \\
& & & \sum_{t=1}^T z_{i,t} \le B_i \ \text{for}\  i\in [m]\setminus S^*\,.
\label{eqn:stackelberg}
\end{aligned}
\end{equation*}
\fi

Our goal is to analyze the robustness of existing CMAB algorithms under the strategic setting and propose strategic variants that guarantee better performance.


==> WSDM/intro.tex <==
Sequential learning methods  feature prominently in a range of real applications such as online recommendation systems, crowdsourcing systems, and online influence maximization problems. Among those methods, the multi-armed bandits problem serves as a fundamental framework. Its simple yet powerful model characterizes the dilemma of exploration and exploitation which is critical to the understanding of online sequential learning problems and their applications to real applications \citep{10.2307/2332286, Robbins:1952,auer2002finite,lattimore_szepesvari_2020}.
The model describes an iterative game constituted by a bandit algorithm and many arms. The bandit algorithm is required to, through a horizon $T$, choose an arm to pull at each time step. As the objective is to maximize the cumulative reward over time, the algorithm balances between exploiting immediate rewards based on the information collected or pulling less explored arms to gain more information about arms \citep{anantharam_asymptotically_1987,auer_nonstochastic_2002,cesa-bianchi_prediction_2006}. % One of the motivating examples to showcase the natural adaptation of MAB to real applications can be recommender systems. The bandits arms may refer to items to be recommended and the bandit algorithm, the recommender system, seek to maximize the cumulative rewards which can be measured through a range of metric. In the simplest case, the rewards can be measured through the number of clicks given by the users and a higher rate of clicking would deem beneficial to the system. 

%Many real applications involve bandit algorithms in their decision systems, including recommendation systems, medical trials, network routing, crowdsourcing systems, combinatorial optimization, automated machine learning, etc.

Out of the real applications, many motivate the extension of MAB towards combinatorial multi-armed bandits (CMAB), where multiple arms can be selected in each round \citep{pmlr-v28-chen13a,DBLP:conf/nips/CombesSPL15,pmlr-v48-lif16,pmlr-v97-zimmert19a,pmlr-v117-rejwan20a}. CMAB demonstrates its effectiveness on problems like online social influence maximization, viral marketing, and advertisement placement, within which many's offline variants are NP-hard. However, existing MAB and CMAB algorithms are often developed either under benign assumptions on the arms \citep{pmlr-v28-chen13a,pmlr-v38-kveton15,pmlr-v75-wei18a} or purely adversarial arms \citep{auer2002nonstochastic}. In the former setting, the arms are commonly assumed to report their reward signals truthfully without any strategic behavior, under which the drawbacks are apparent.

In the later setting, arms can attack any deployed algorithm to a regret of $O(T)$ with this capability of reward manipulations, which is catastrophic for a bandit algorithm. 
This assumption is stringent and rarely realistic.

In this paper, we first rigorously analyze the difference between the assumptions placed on the adaptive arms and the regret upper and budget lower bounds thereof, in both MAB and CMAB. 
These justify our intuition that strategic manipulation is indeed a weaker assumption on arms' influence on the regret.
To put forward a bandit algorithm under strategic arms, we adapt the combinatorial UCB (CUCB) algorithm with a carefully designed UCB-based exploration term. 
A major difficulty stems from not knowing the manipulation term made by the arms, while our algorithm overcomes this by depending only on the knowledge of the maximum possible strategic budget.
New tail bounds over the proposed exploration term and a new trade-off parameter that balances exploration and exploitation are utilized to facilitate the analysis of our algorithm.
We further establish results on the robustness of our UCB variant under strategic arms with an algorithm-dependent budget lower bound.

Our proposed algorithms are also evaluated empirically through an extensive set of synthetic environments and real datasets. 
The real applications include reliable workers selection in online crowdsourcing systems, where workers might misrepresent a result for a better chance to be selected in the future; online information maximization, where nodes modify the spread to include itself into the seed set; and online recommendation systems, which characterizes the ``click framing'' behavior. Through a wide range of tasks and parameters, the experiment results corroborate our theoretical findings and demonstrate the effectiveness of our algorithms.

\subsection{Motivating Examples}
\input{motivation}



==> WSDM/lower.tex <==
To fully understand the effects of strategic manipulations, we investigate the relationship between the strategic budget and the performance of UCB-based algorithms. Our results provide the dependency between an arm's strategic budget and the number of times it is pulled, which influence the regret of the algorithm incurred by the arm. Our analysis gains some insight from \citet{zuo_near_2020}, which limits the discussion to the 2-armed bandit setting and cannot be applied to the general MAB setting directly. 

%Counter-intuitively, the dependency between the number of pulls of a strategic arm and its strategic budget is linear and subsequently, this infers that the regret depends on each strategic budget linearly.
%For a strategic arm to manipulate the algorithm to suffer an undesired regret of $\omega(k)$, where $k\ge O(\log T)$, the strategic budget must be at least $\omega(k)$.
%We formalize this statement in Theorem \ref{lower}, while we defer the complete proof to the appendix.

We first define some notations used in the theorem.
Without loss of generality, let arm $i^{\ast}$ be the optimal arm and arm $i, i \neq i^{\ast}$ be an arbitrary strategic suboptimal arm. Assume that arm $i$ has no access to the information regarding other arms. Let $K_{i,t}$ and $K_{i^{\ast},t}$ denote the number of times arm $i$ and arm $i^{\ast}$ have been pulled up to time $t$, respectively. Denote $\hat{\mu}_{i,t}$ as the empirical estimate of the underlying mean $\mu$ without manipulations, i.e., $\hat{\mu}_{i,t} = \frac{\sum^{t-1}_{j=1}x_{i,j}}{K_{i,t-1}}$. Define the suboptimality gap for each strategic arm $i$ to be $\delta_i = \mu_{i^{\ast}} - \mu_i$. We use a slightly revised UCB algorithm as the basic algorithm, where the UCB estimation term for arm $i$ is $\hat{\mu}_{i,t} + \sqrt{\frac{2\log(K_{i,t}^2/\eta^2)}{K_{i,t}}}$ and $\eta$ is a confidence parameter chosen by the algorithm.

\begin{theorem}\label{lower}
In stochastic multi-armed bandit problems, for a strategic suboptimal arm $i$ without access to other arms' information, to be pulled for $\omega(k)$ in $T$ steps under the UCB algorithm where $k\ge O(\log{T})$, the minimum strategic budget is $\omega(k)$. 
%The regret incurred is thus $\omega(\log{T})$. 
\end{theorem}

\iffalse
\begin{proof}[Proof sketch] 
Let $t \in [1,T]$ be the time step arm $i$ is pulled for the last time, the following inequality must stand
\begin{align*}
& \hat{\mu}_{i,t} + \sqrt{\frac{2\log(K_{i,t}^2/\eta^2)}{K_{i,t}}} + \frac{\rho_i}{K_{i,t}}\geq \hat{\mu}_{i^{\ast},t} + \sqrt{\frac{2\log(K_{i^{\ast},t}^2/\eta^2)}{K_{i^{\ast},t}}}\,.
\end{align*}
By the Chernoff-Hoeffding bound and the union bound, 
\begin{align*}
\quad \mathbb{P} \left(\hat{\mu}_{i,t}  - \mu_i  \geq \sqrt{\frac{2\log(K_{i,t}^2/\eta^2)}{K_{i,t}}}\right) \leq  \frac{\pi^2}{6} \eta^2 \,.
\end{align*} 
Hence, with probability $1 - 2 \frac{\pi^2}{6}\eta^2$, we have %$(1 - \eta^2 \frac{\pi^2}{6})^2$, 
\begin{align}
\mu_i + \sqrt{\frac{2\log(K_{i,t}^2/\eta^2)}{K_{i,t}}} + \frac{\rho_i}{K_{i,t}} \geq \mu_{i^{\ast}}\,. \notag
\end{align}
When arm $i$ is pulled, arm $i$ wants to ensure the following holds
\begin{align}
 \sqrt{\frac{2\log(K_{i,t}^2/\eta^2)}{K_{i,t}}} + \frac{\rho_i}{K_{i,t}} \geq \delta_i\,,\notag
\end{align}
where $\delta_i = \mu_{i^{\ast}} - \mu_i$. Then,
\begin{equation*}
B_i \geq \rho_i \geq \left(\delta_i - \sqrt{\frac{2\log(K_{i,t}^2/\eta^2)}{K_{i,t}}}\right) \cdot K_{i,t}\,.  \qedhere
\end{equation*}
\end{proof}
\fi 
This dependency of $k$ can be extended to CMAB and CUCB straightforwardly when arms within an arm subset collude. Counter-intuitively, the dependency between the number of pulls of a strategic arm and its strategic budget is linear and subsequently, this infers that for a strategic arm to manipulate the algorithm to suffer an undesired regret of $\omega(k)$, where $k\ge O(\log T)$, the strategic budget must be at least $\omega(k)$.

==> WSDM/motivation.tex <==
The setting of strategic manipulations describes the strategic behavior found in a variety of real applications. We discuss two popular applications in details, namely workers selection in online crowdsourcing platforms and online influence maximization through social networks. 

\subsection{Online Worker Selection in Crowdsourcing Platforms}

Consider a crowdsourcing platform that provides data labelling service for a payment. The platform interact with a group of customers and a pool of workers. The customers request tasks to the platform for labeling and the platform is then responsible of selecting workers from the worker pool to complete the tasks. This process repeats, during which the platform learns the best deployment. We maintain a mild assumption that the payments from customers are non-decreasing with the quality of labels. To maximize its profit, it is desired for the platform to select workers that provides most reliable labels. The workflow of the platform can be described in the diagram below. %\ref{crowdsys}. 

While the platform and the customers desire quality labels, it may not entirely be in the worker's interest to exert highest effort and thus report quality labels each time, which factors into a range of reasons. Workers may adapt strategic behaviors to maximum their own utility instead. Thus, it becomes crucial to identify the reliable workers to prevent strategic behaviors that jeopardize profits.
This naturally translate to a combinatorial multi-armed bandits problem under strategic manipulations where the workers are the strategic arm and the payments acts as the rewards.

\begin{figure}[H]
\centering
\label{crowdsys}
\includegraphics[width=7.5cm]{figs/crowdsys.png}
\caption{Online crowdsourcing system}
\end{figure}

\subsection{Online Influence Maximization}

For a social network that can be represented by the below directed graph where white dots are people and black dots labeled with ``SI'' are social influencers. The temporal nature of social network results in each directed edges exists with a probability at each time step. Formally, a node is said to be reached by a seed node if there it has a directed path from the seed node. Note that this definition considers a diffusion process where a node can be reached by a seed node through multiple edges. Given a set of seed nodes, we define a spread across social network at a given time $t$ by the expected number of nodes that can be reached by the nodes in the seed node set at that time. Intuitively, this models information spread among social networks and reflects scenarios like viral marketing.

\begin{figure}[H]
\centering
\includegraphics[scale = 0.35]{figs/example.png}
\caption{Probabilistic social network}
\end{figure}

In the case of product marketing, a company may need to select the most influential social influencers to collaborate with to maximize the expected spread across time. This can be expressed as an online influence maximization problem as the company seek to maximize the size of population reached by promotions across number of promotions. However, in many cases social influencers may report inaccurate information regarding their social influential ability, which may corresponds to a number of ways in real applications, such as faking follower numbers on social media platforms. 


==> WSDM/related.tex <==

\iffalse
\begin{table*}[t]
\begin{tabular}{|c|c|c|c|c|}
\hline
\multicolumn{5}{|c|}{Problem Formulation}                                                                             \\ \hline
\multicolumn{1}{|l|}{}                                        
& \begin{tabular}[c]{@{}c@{}}Pure\\ Adversarial\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}Adversarial \\ Attack\end{tabular}                                  
& \begin{tabular}[c]{@{}c@{}}Adversarial \\ Corruption\end{tabular}                                  
& \begin{tabular}[c]{@{}c@{}}Strategic\\ Manipulations\end{tabular}                                                     \\ \hline
\begin{tabular}[c]{@{}c@{}}Budget \\ constraints\end{tabular} & None                                                  & \begin{tabular}[c]{@{}c@{}}Group\\ constraints\end{tabular}                                    
& \begin{tabular}[c]{@{}c@{}}Group\\ constraints\end{tabular}                                        
& \begin{tabular}[c]{@{}c@{}}Individual\\ constraints\end{tabular}                                                    \\ \hline
Objective                                                     
& Unspecified                                                
& \begin{tabular}[c]{@{}c@{}}Group\\ interest\end{tabular}                                       
& \begin{tabular}[c]{@{}c@{}}Group\\ interest\end{tabular}                                           
& \begin{tabular}[c]{@{}c@{}}Individual \\ interest\end{tabular}                                                      \\ \hline
Regret        
& $O(\sqrt{T})$  \citep{NIPS2014_25b2822c}
& \begin{tabular}[c]{@{}c@{}}Attack cost of $O(\log T)$ \\ with $\omega(T)$ regret \\ \citep{NEURIPS2018_85f007f8}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}Identify best arm with up to\\  $O(\sqrt{T/K})$ corruption \\ \citep{pmlr-v99-gupta19a}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}$O(\log T)$  \\ \citep{pmlr-v119-feng20c}\end{tabular} \\ \hline
\end{tabular}
\caption{\label{tab:summary}Summary of various bandit problems.}
\end{table*}
\fi

The problem of multi-armed bandits (MAB) was first investigated back to 1952 while some techniques utilized was developed back to 1933 \citep{10.2307/2332286, Robbins:1952, berry,auer2002finite,lattimore_szepesvari_2020}. Since then it has been extensively explored and serves as the foundation of many modern areas, including reinforcement learning, recommendation systems, graph algorithms, etc. \citep{DBLP:conf/iconip/BouneffoufBG12,pmlr-v70-vaswani17a, pmlr-v85-durand18a, li2020stochastic}. With the need to model the selection of multiple arms in one round, MAB is then extended to combinatorial multi-armed bandits (CMAB), %The latter, despite being more complicated to analyze and implement, covers a richer set of settings and has a better synergy with offline approximation algorithms who can be used as oracles. CMAB algorithms 
which see many deployments in real applications like news/goods recommendation, medical trials, routing, and so forth \citep{Wang_Ouyang_Wang_Chen_Asamov_Chang_2017,8022964,pmlr-v84-sankararaman18a, li2020online}. 

%Though many studies focus on stochastic MAB and stochastic CMAB, which are the vanilla settings that the rewards of arms are independent and drawn from stationary distributions, 
Real applications motivate the community to derive algorithms in more adaptive environments.% compare to the vanilla settings that the rewards of arms are independent and drawn from stationary distributions. 
The first of which considers adversarial bandits with the classic EXP3 algorithm. The arms are assumed to be non-stationary but non-adaptive (which means that algorithms will adapt to the adversarial) \cite{auer2002nonstochastic}. Despite that adversarial bandits do not fall under the scale of this paper's related work, it leads tremendous effort to the following topics in adaptive arms.% and it is technically the Lagrangian dual of bandits with adversarial corruptions.

\paragraph{Adversarial corruptions}
%Adversarial corruption in bandits is a form of adaptive reward that poses relatively the largest difficulty for bandit algorithms. 
The adversary is given the ability to replace the observations of the bandit algorithm with arbitrary values within some constraints.
\citet{pmlr-v99-gupta19a} discuss the constraint that rewards are modified for at most $T_0$ rounds out of the total $T$ rounds. The asymptotic regret bound $O(mT_0)$ achieved in the work is shown to match the negative result, where $m$ is the number of arms. \citet{lykouris_stochastic_2018} discussed a different constraint where the corruption $z_t$ at time $t$ is cumulative up to some constant $B$%, which writes $\sum^T_{t=1} z_t \leq B$. 
The regret achieved under this constrained corruption is bounded by $O(mB\log(\frac{mT}{\delta}))$ with probability at least $1 - \delta$. \citet{JMLR:v20:18-395} restricts corruptions as independent Bernoulli events with probability $b$, while if corruption happens the reward becomes arbitrary and adversarial. This problem is addressed with median statistics with gap-dependent matching regret upper and lower bounds of $O(\sum_{i \neq i^{\ast}} \frac{1}{\Delta_i}\log(\frac{K}{\Delta_i}))$, where $i^{\ast}$ denotes the optimal arm and $\Delta_i$ is the suboptimality of arm $i$.

Several lines of research also discuss corruption topics in frequentist inference and partial monitoring \citep{pmlr-v83-gajane18a}, best arm identification \citep{pmlr-v99-gupta19a}, and adversarial bandits \citep{NEURIPS2020_e655c771}.

\paragraph{Adversarial attacks}
Different from arms in adversarial corruptions who intend to maximize the regret of the bandit algorithm, arms in the adversarial attack setting have the goal to maximize their number of pulls. 
%The objectives of the bandit algorithm and the arms do not agree in general, but they are not completely opposite either. 
The setting is first considered by \citet{NEURIPS2018_85f007f8}, where it shows that the attacker may spend a budget of $O(\log T)$ to deceit UCB and $\epsilon$-greedy algorithms to pull the target arms for at least $T - o(T)$ times. Stochastic and contextual MAB algorithms also suffer from undesired loss from this adversarial attack, under a variety of attack strategies \citep{pmlr-v97-liu19e}. Linear MAB algorithms, however, are shown to be near-optimal up to some linear or quadratic terms on the attack budget $B$ \citep{garcelon_adversarial_2020,bogunovic_stochastic_2020}. 

\paragraph{Strategic manipulations}
The setting of strategic manipulations further weakens the capability of the adaptive arms and prevents the bandit algorithms from being overcautious. 
The objective of an arm is still utility maximization under strategic manipulations, while each arm works on its utility individually. 
Instead of having a global coordinator for the adversarial attack strategy, the strategic arms seek the best response via the dominant Nash equilibrium. 
The strategic manipulation setting is first studied by \citet{pmlr-v99-braverman19b} where each arm is assumed to keep portion of the reward in each round and arms maximize the cumulative reward it keeps. 
The performance of bandit algorithms will then be catastrophic under the dominant Nash equilibrium, receiving an expected cumulative reward of $0$ almost surely. 
With the utility of maximizing the number of pulls for each strategic arm, common bandits algorithms are proved to be robust with guaranteed $O(\log T)$ regret bound, but only under constant strategic budgets \citep{pmlr-v119-feng20c}. 
For $\omega(\log T)$ budgets, bandits under strategic manipulations remain an open problem and will be discussed in this paper. 

%\citet{pmlr-v119-feng20c} is the first to study regret minimization under the strategic bandit setting. The work investigated various classical bandit algorithms, such as UCB, $\epsilon$-greedy and Thompson Sampling, and certify the robustness of these algorithms with a regret of $O(\log T)$. However, the lower bound presented in the work is logarithmic dependent and become vacuous when B is of $O(\log T)$


==> WSDM/strategy.tex <==
%There exists a range of assumptions on the underlying stochastic game in the multi-armed bandit frameworks. On one extreme of the spectrum is the adversarial bandit problem, where the algorithm observes rewards that are presumed to be chosen by an adversary. On the other extreme, we have the stochastic bandit problem where the observed rewards generated by each arm are associated with a stationary distribution. Most real applications, however, fall somewhere on this spectrum in between the extreme points. Previous works on bandit problems with adversarial attack \citep{NEURIPS2018_85f007f8,pmlr-v97-liu19e,garcelon_adversarial_2020,bogunovic_stochastic_2020}, adversarial reward corruptions \citep{lykouris_stochastic_2018,pmlr-v99-gupta19a,JMLR:v20:18-395}, and strategic manipulations \citep{pmlr-v99-braverman19b,pmlr-v119-feng20c} aim to give the most suitable descriptions of the real problems. 

From a game-theoretical point of view, %the optimal collusion strategy of bandit arms serves as a bridge towards different acknowledgments of arms' individual interests. 
by considering collusion, we can reduce the underlying bi-levels stochastic game in bandits with strategic manipulations to a two-party game with the learning algorithm and the arms and thus have a standard to gauge the performance of algorithms along with the hardness of each bandit problems. This positions the setting of strategic manipulations among existing settings like adversarial corruptions and adversarial attacks.

%We start by discussing the optimality of the lump sum investing (LSI) strategy, the subgame perfect dominant strategy, under collusion. 
%Despite that \citet{pmlr-v119-feng20c} prove the subgame dominance among arms of lump sum investing (LSI) strategy, 
We present a counter-example where the subgame dominant strategy the lump sum investing (LSI) strategy is suboptimal when the arms collude \citet{pmlr-v119-feng20c}. % under the common goal of regret maximization. 
Consider a three arms bandit instance with mean $\mu, \mu - \Delta, \mu - 2\Delta$ expected rewards, respectively. 
With the UCB algorithm, the first three time steps are for initialization where the algorithm pulls each arm once. 
%Clearly, any strategy is an optimal collusion strategy for the time horizon of $T = 1, 2, 3$. 
When the time horizon $T$ is $4$, however, the optimal strategy would lure the algorithm to pick arm 3 at time step 4. 
This objective is achieved when arm 3 spends all of its strategic budgets whenever it is first pulled and lets arm 2 be truthful about its emitted rewards. 
Under the LSI strategy, both arm 2 and arm 3 would spend all of their strategic budgets when they are first pulled, which happens in the initialization rounds.
%When the time horizon $T=5$, the optimal collusion strategy becomes letting arm 3 spends all of its budgets when it is first pulled, letting arm 2 spends $\Delta$ when it is first pulled, and spends the rest of its budget on its second pull. Under this strategy, arm 3 is guaranteed to be pulled at time step 4 if it possesses enough strategic budgets to alter rewards higher than the optimal arm is capable of. As arm 2 spends $\Delta$, which is exactly the suboptimality gap, arm 2 is just as good as the optimal arm at a time step of 5. 

We then establish a portrayal of the optimal collusion strategy by formulating the problem into a combinatorial optimization problem. % under the goal of maximizing the number of suboptimal pulls. 
%It is a similar formulation with the regret maximization problem our counter-example is built on, which will be deferred to the appendix. 
%Extensive empirical results on the optimality of variants of LSI as collusion strategies are also discussed in the appendix.
%but under the objective of maximizing regret along with 

%\subsection{Suboptimal pulls maximization}
\begin{claim}
Under a strategic stochastic multi-armed bandit problem, when the strategic suboptimal arms collude to maximize the number of suboptimal pulls of the UCB algorithm with confidence parameter $\sqrt{\frac{3\log t_i}{K_{i,t-1}}}$, the maximum number of suboptimal pulls is the solution of 
\begin{equation*}
\begin{aligned}
& \underset{Y_{i},t_i,\ i\in [m]}{\mathrm{maximize}}
& & Y_{1}+\dots+Y_{m} \\
& \mathrm{subject}\text{ }\mathrm{to}
& & \frac{B_i}{Y_{i}} + \sqrt{\frac{3\log t_i}{Y_{i}}} \ge \delta_i + \sqrt{3\log t_i},\ i \in [m]\,, \\
& & &  t_{i_j} \ge \sum_{l=1}^j Y_{i_l}, \ j\in [m]\,,\\
& & &  \textup{for some permutation}\ i_1,\dots\ i_m\ \textup{of}\ [m]\,.\\
\end{aligned}
\end{equation*}
%\begin{align*}
%&\textup{maximum} \ K_{1,T}+\dots+K_{m,T}\\
%& \textup{subject to} \ \ \frac{B_i}{K_{i,t-1}} + \sqrt{\frac{3\log t_i}{K_{i^,t-1}}} \ge \delta_i + \sqrt{3\log t_i},\ i \in [m] \\
%&\text{there exists a permutation}\ \ i_1, \dots, i_{m-1}\\
%&t_{i_1} \ge K_{i_1}\\
%&t_{i_2} \ge K_{i_1} + K_{i_2}\\
%&\dots \\
%&t_{i_{m-1}} \ge K_{i_1} + \dots + K_{i_{m-1}}\\
%\end{align*}
\end{claim}
In the program, $Y_i$ represents the total number of times arm $i$ is pulled, which corresponds to $K_{i,T-1}$ used in previous sections. The permutation $i_1,...,i_m$ then describes, before the optimal arm is first pulled, the chronological order of the suboptimal arms to complete their last pull.
Observe that the confidence parameter of the optimal arm %$\frac{B_i}{K_{i,t-1}} + \sqrt{\frac{3\log{t}}{K_{i,t-1}}} - \sqrt{\frac{3\log{t}}{K_{i^{\ast},t-1}}}$ 
increases with respect to $t$, the inequality holds for $t_i$ if and only if it holds for all $t\le t_i$.
%With the constraint that the total number of pulls must not exceed the time index.%, we obtain the complete combinatorial program.
%The above-mentioned assumption is natural for the optimal strategy under collusion. Intuitively, two suboptimal arms should not be `competing' to get pulled. In other words, the optimal strategy ensures that the inequality stands for one suboptimal arm $i \in [m]$ uniquely. The optimal strategy search for a permutation $i_1,...,i_m$, which $i_j$ describes the last time where a strategic arm $j$ is pulled.
%Under the UCB algorithm, a suboptimal arm $i, i \neq i^{\ast}$ is pulled if and only if the following inequality stands
%\begin{align*}
%     \frac{B_i}{K_{i,t-1}} + \sqrt{\frac{3\log(t)}{K_{i,t-1}}} \geq \delta_i + \sqrt{\frac{3\log(t)}{K_{i^{\ast},t-1}}}\,.
%\end{align*}
%Hence the search for optimal collusion strategy is equivalent to the search for a combination of arms spending budgets to optimize the number of times the inequality holds. As $K_{1,T}+\dots+K_{m,T}$ records the number of times this inequality is true, the combinatorial optimization objective can be written in terms of maximizing $K_{1,T}+\dots+K_{m,T}$.
By the same observation that the advantage of the optimal arm increases with time, %it is, therefore, in a bandit arm's best interest to spend its strategic budget as early as possible. 
%Based on this observation, 
strategic arms who optimally spend their budgets for the maximum amount of pulls will also maximize their number of pulls till the first optimal arm pull. 
The inequality condition of the combinatorial program is thus $\frac{B_i}{K_{i,t-1}} + \sqrt{\frac{3\log t_i}{K_{i,t-1}}} \ge \delta_i + \sqrt{3\log t_i}$. 
We term the class of approximately optimal strategy as `sequential pull strategy', in which the strategic arms deceit the learning algorithm to pull suboptimal arms until the depletion of the budgets and this class includes the LSI strategy.

%The inequality $\frac{B_i}{K_{i,t-1}} + \sqrt{\frac{3\log t}{K_{i,t-1}}} \ge \delta_i + \sqrt{\frac{3\log t}{K_{i^{\ast},t-1}}}$ is a necessity for arm $i$ to be pulled, and will be sufficient under the assumptions that no suboptimal arms compete for the pulls. This condition translates to the case where the inequality does not simultaneously hold for two suboptimal arms. We conjecture that the condition must hold for some optimal strategy by carefully designing the initial budget commitments. When the condition holds, the inequality term $t_{i_j} \ge \sum_{l=1}^j Y_{i_l}$ can then be relaxed to an equality $t_{i_j} = \sum_{l=1}^j Y_{i_l}$.

%Knowing this, we build the intuition that the search for optimal collusion strategy lay on the search of optimal order of budget spending, in accordance to some priorities dependent of arm's background information and optimization objective.

==> strategic combinatorial WSDM/WSDM/algoproof.tex <==

We now propose a variant of combinatorial upper confidence bound algorithm that is robust to strategic manipulations of rewards in Algorithm \ref{algo}. The only mild assumption we maintain is that the learning algorithm has the knowledge of the largest budget possessed among all bandits arms, i.e, $B_{max}$. This is a relaxation of the assumptions made by \citet{pmlr-v119-feng20c} on strategic UCB algorithm, in which the learning algorithm has access to the cumulative use of budget at every time step. We start with a detailed description of the algorithm and then analyze the theoretical upper bound of regret, which enjoys $O(m \log{T} + m B_{max})$. 

For each arm $i$, our algorithm maintains a counter $K_{i,t-1}$ as the total number of times arm $i$ has been pulled up to time $t-1$ and $\widetilde{\mu}_{i,t} = \frac{\sum_{j=1}^{t-1} (x_{i,j}+ z_{i,j})}{K_{i,t-1}}$ as the empirical mean estimation based on the observations. At each time step, the algorithm computes the UCB estimation $\Bar{\mu}_{i,t}= \widetilde{\mu}_{i,t} + \sqrt{\frac{ 3 \log{t} }{2K_{i,t-1}}} + \frac{B_{max}}{K_{i,t-1}}$ for $i \in [m]$. With $\Bar{\mu}_{i,t}$, the $(\alpha, \beta)$-approximation oracle then outputs an approximately optimal arm subset $S_t \in \mathcal{S}$. The algorithm plays the return arm subset and update the counter $K_{i,t}$ and the estimation $\widetilde{\mu}_{i,t}$ accordingly. 

\begin{algorithm}[htb]
\DontPrintSemicolon
{\bf Input:}
Horizon $T$, number $m$ of arms, maximum budget $B_{max}$\;
{\bf Output:} Arm subset $S_t$\; 
  Initialize $K_{i,0} = 0$ and $\widetilde{\mu}_{i,0} = 0$ for $i \in [m]$\; 
  \For{t = 1 $\to$ m}{
    Play an arbitrary arm subset $S_t \in \mathcal{S}$ such that $t \in S_t$\; 
    $K_{i,t} = K_{i,t-1} + 1$ for $i \in S_t$\;
    $\widetilde{\mu}_j = x_{i,t}+z_{i,t}$ for $i \in S_t$ \;}
  \For{t = m+1 $\to$ T}{
  For $i \in [m]$, compute $\Bar{\mu}_{i,t}= \widetilde{\mu}_{i,t-1} + \sqrt{\frac{ 3 \log{t} }{2K_{i,t-1}}} + \frac{B_{max}}{K_{i,t-1}} $\;
  $S_t$ = {\textbf{oracle}}$(\Bar{\mu}_{1,t},\Bar{\mu}_{2,t},.....,\Bar{\mu}_{m,t})$\;
  Play arm subset $S_t$ and update 
  $K_{i,t} = K_{i,t-1} + 1$ and $ \widetilde{\mu}_{i,t} =  \frac{\sum_{j=1}^{t} (x_{i,j} + z_{i,j})}{K_{i,t}}$ for $i \in S_t$ \;
  }
\caption{SCUCB}
\label{algo}
\end{algorithm}

We first introduce a few notations that are used in our results. Define, for any arm $i\in[m]$, the suboptimality gaps as
\begin{align*}
        &\Delta^i_{min} = \alpha \cdot {OPT}_{\bm{\mu}} - \max\{r_{\bm{\mu}}(S) \mid S \in S_B, i \in S\}\,, \notag \\
     &\Delta^i_{max} = \alpha \cdot {OPT}_{\bm{\mu}} - \min\{r_{\bm{\mu}}(S) \mid S \in S_B, i \in S\}\,.
\end{align*}
We then denote the maximum and minimum of the suboptimality gaps as $\Delta_{max} = \max_{i \in [m]} \Delta^i_{max}\notag $ and $\Delta_{min} = \min_{i \in [m]} \Delta^i_{min}$.

The following lemma re-establish the canonical tail bound inequality in UCB under the setting of strategic manipulations. %The complete proof of Lemma \ref{lambda} is deferred to the appendix.
\begin{lemma}\label{lambda}
Let ${\Lambda}_{i,t} = \sqrt{\frac{3 \log{t} }{2K_{i,t-1}}} + \frac{\rho_{i,t-1}}{K_{i,t-1}}$, where $\rho_{i,t-1}$ is the total strategic budget spent by arm $i$ up to time $t-1$ and $K_{i,t-1}$ be the total number of pulls of arm $i$ up to time $t-1$. Define the event $E_t = \{ |\ \widetilde{\mu}_{i,t-1} - \mu_{i}| \leq \Lambda_{i,t}, \forall i \in [m]\}$, where $\mu_i$ is the true mean of arm $i$'s underlying distribution. 
Then, $\mathbb{P}(\lnot E_t)\leq 2m \cdot t^{-2}$.
\end{lemma}
\iffalse
\begin{proof}[Proof sketch] 
Denote $\hat{\mu}_{i,t-1} = \frac{\sum_{j=1}^{t-1} x_{i,j}}{K_{i,t-1}}$ as the estimation of the expected reward without the manipulated variable $z_{i,t}$. By the definition of $\hat{\mu}_{i,t}$ and $\widetilde{\mu}_{i,t}$,
\begin{align}
& \mathbb{P}\left(|\widetilde{\mu}_{i,t-1} - \mu_i| > \sqrt{\frac{3\log{t}}{2K_{i,t-1}}} + \frac{\rho_{i,t-1}}{K_{i,t-1}}\right) \notag \\
    %=\ & \mathbb{P}\left(\left|\hat{\mu}_{i,t-1} + \frac{\rho_{i,t-1}}{K_{i,t-1}}- \mu_i\right| > \sqrt{\frac{3\log{t}}{2K_{i,t-1}}} + \frac{\rho_{i,t-1}}{K_{i,t-1}} \ \right) \notag \\
    \leq\ & \mathbb{P}\left(\hat{\mu}_{i,t-1} - \mu_i > \sqrt{\frac{3\log{t}}{2K_{i,t-1}}} \ \right) + \mathbb{P}\left(\hat{\mu}_{i,t-1} - \mu_i <  -\sqrt{\frac{3\log{t}}{2K_{i,t-1}}}\right) \notag \\
    \leq\ & \sum_{s=1}^{t} \mathbb{P}\left(|\hat{\mu}_{i,{t-1}} - \mu_i|  > \sqrt{\frac{3\log{t}}{2s}}\ \right)\notag\\
    \leq\ & 2t\cdot \exp{(-3\log{t})} = \frac{2}{t^2} \,,\notag
\end{align}
where the last inequality follows the Chernoff-Hoeffding bound. By the union bound,
\[
\quad \mathbb{P}(\lnot E_t) = \mathbb{P}\left( \{ \forall i \in [m] ,\ |\widetilde{\mu}_{i,t-1} - \mu_{i}| > \Lambda_{i,t}\} \right)\leq 2m \cdot t^{-2} \,. \qedhere
\]
\end{proof}
\fi

Armed with Lemma \ref{lambda}, we present one of our main theorems, Theorem \ref{appendixA}, which gives the regret bound of $O(\log T)$ of SCUCB. The outline of the proof follows that of CUCB by \citet{pmlr-v28-chen13a}. To complete the proof, we carefully choose $\psi_t$, which controls the trade-off between the exploration and exploitation periods.% The full proof is deferred to the appendix.

\begin{theorem}
\label{appendixA}
The regret of the SCUCB algorithm with $m$ strategic arms in time horizon $T$ using an $(\alpha,\beta)$-approximation oracle is at most 
\begin{align}
 m\cdot\Delta_{max}\left( \frac{8B_{max} f^{-1}(\Delta_{min}) + 6\log{T}} {\left(f^{-1}(\Delta_{min})\right)^2} + \frac{\pi^2}{3}+1 \right)\,, \notag \nonumber
\end{align}
where $f^{-1}(\cdot)$ is the inverse bounded smoothness function.
\end{theorem}

\begin{proof}[Proof sketch]
We introduce a counter $N_i$ for each arm $i\in[m]$ after the $m$-round initialization and let $N_{i,t}$ be the value of $N_i$ at time $t$. We initialize $N_{i,m} = 1$. By definition, $\sum_{i \in [m]} N_{i,m} = m$. For $t > m$, the counter $N_{i,t}$ is updated as follows:
\begin{itemize}
    \item If $S_t \in S_B$, then $N_{{i'},t} = N_{{i'},t-1} + 1$ where $i' =$ $\argmin_{i \in S_t}$ $N_{i,t-1}$. In the case that $i'$ is not unique, we break ties arbitrarily;
    \item If $S_t \notin S_B$, then no counters will be updated. 
\end{itemize}  
As such, the total number of pulls of suboptimal arm subsets is less than or equal to $\sum_{i=1}^m N_{i,T}$.

Define $\psi_t = \frac{8B_{max}f^{-1}(\Delta_{min}) + 6\log{t}} {\left(f^{-1}(\Delta_{min})\right)^2} > c $, where $c$ is the larger solution of
\begin{align*}
\label{square}
    &(f^{-1}(\Delta_{min}))^2 c^2  + 16B_{max}^2 - ((8B_{max} f^{-1}(\Delta_{min})- 6\log{t}) c = 0 \,. %\notag
\end{align*}
%We use $\mathbb{I}\{\cdot\}$ to denote the indicator function, and $\mathbb{I}\{A\}$ is 1 if event $A$ is true and 0 otherwise. 
Then, we decompose the total number $\sum_{i=1}^m N_{i,T}$ of pulls of suboptimal arm subsets as
\begin{align}
\sum_{i=1}^m N_{i,T} = \ & m +\sum_{t=m+1}^T \mathbb{I}\{ S_t \in S_B\} \notag \\
=\ &m +\sum_{t=m+1}^T \sum_{i=1}^m \mathbb{I}\{ S_t \in S_B, N_{i,t} > N_{i,t-1}, N_{i,t-1} \leq \psi_t\} \notag \\
&+ \sum_{t=m+1}^T \sum_{i=1}^m \mathbb{I}\{ S_t \in S_B, N_{i,t} > N_{i,t-1}, N_{i,t-1} > \psi_t\}\notag \\
\leq \ & m + m\psi_T+\sum_{t=m+1}^T \mathbb{I}\{ S_t \in S_B,N_{i,t-1} > \psi_t, \forall i \in S_t\}\,. \notag
\end{align}

The inequality follows as $\sum_{t=m+1}^T \sum_{i=1}^m \mathbb{I}\{ S_t \in S_B, N_{i,t} > N_{i,t-1}, N_{i,t-1} \leq \psi_t\}$ can be trivially bounded by $m\psi_T$. Thus the key to bound the total number of pulls of suboptimal arm subset is to upper bound $\sum_{t=m+1}^T \mathbb{I}\{ S_t \in S_B,N_{i,t-1} > \psi_t, \forall i \in S_t\}$. Let $F_t$ denotes the event that the oracle fails to provide an $\alpha$-approximate arm subset with respect to the input vector $\Bar{\bm{\mu}} = (\Bar{\mu}_{1,t},\Bar{\mu}_{2,t},.....,\Bar{\mu}_{m,t})$. 
Then we can decompose $\sum_{t=m+1}^T \mathbb{I}\{ S_t \in S_B,N_{i,t-1} > \psi_t, \forall i \in S_t\}$ as 
\begin{align}
&\quad \sum_{t=m+1}^T \mathbb{I}\{ S_t \in S_B,N_{i,t-1} > \psi_t, \forall i \in S_t\}\notag\\
%&\leq \sum_{t=m+1}^T (\mathbb{I}\{F_t\} + \mathbb{I}\{ \lnot F_t, S_t \in S_B,N_{i,t-1} > \psi_t, \forall i \in S_t\})\notag\\
&\leq \sum_{t=m+1}^T (\mathbb{I}\{F_t\} + \mathbb{I}\{ \lnot F_t, S_t \in S_B,  K_{i,t-1} > \psi_t, \forall i \in S_t\})\notag \\
&\leq (T-m)(1-\beta) +  \mathbb{I}\{ \lnot F_t, S_t \in S_B, K_{i,t-1} > \psi_t, \forall i \in S_t\}\notag \,. \notag
\end{align}

By leveraging the monotonicity and smoothness assumptions of the reward function, we show that $\mathbb{P}(\{\lnot F_t, E_t,  S_t \in S_B, K_{i,t-1} > \psi_t, \forall i \in S_t\}) = 0$. Therefore, by the inclusion-exclusion principle,
\begin{align}
     \mathbb{P}(\{\lnot F_t, S_t \in S_B, K_{i,t-1} > \psi_t, \forall i \in S_t\}) 
     &\leq \mathbb{P}(\lnot E_t) \leq 2m \cdot t^{-2} \,.\notag
\end{align}
%where the last inequality comes from lemma \ref{lambda}. 

Leveraging the upper bound of total number of pulls of suboptimal arm subsets, the regret is bounded by
\begin{align}
    & \quad Regret_{\bm{\mu},\alpha,\beta}(T)
    \notag \\
    & \leq T\alpha \beta \cdot \text{OPT}_{\bm{\mu}} - \left( T\alpha\cdot \text{OPT}_{\bm{\mu}} - \mathbb{E} \left[ \sum_{i=1}^m N_{i,T} \right]\cdot \Delta_{max} \right)
    \notag \\
     &\leq m\cdot \Delta_{max}\left(\frac{8B_{max} f^{-1}(\Delta_{min}) + 6\log{T}} {\left(f^{-1}(\Delta_{min})\right)^2} + \frac{\pi^2}{3}+1\right)\,. \notag \qedhere
\end{align}
\end{proof}

It remains in question whether a bandit algorithm can achieve a regret upper bound sublinear in $B_{max}$. 
Our conjecture is negative.
In fact, under strategic manipulations of rewards, the design of robust bandit algorithms, e.g. UCB and $\epsilon$-greedy, is analogous to the design of outlier-robust mean estimation algorithms. Existing works on robust mean estimation, such as \citet{steinhardt_et_al:LIPIcs:2018:8368}, argue that, from an information theoretical point of view  mean estimation error must be depending on the variance of the data. Casting this argument to bandit with the strategic manipulation setting, we believe that a tight regret bound is unlikely to be independent of the strategic budget $B_{max}$. Moreover, Proposition 4 in \citet{steinhardt_et_al:LIPIcs:2018:8368} implies that the dependency on $B_{max}$ is linear. This corresponds to our linear dependency of regret in Theorem \ref{appendixA}.


==> strategic combinatorial WSDM/WSDM/exp.tex <==
In this section, we evaluate our SCUCB algorithm empirically on synthetic data and three real applications, namely online worker selection in crowdsourcing, online recommendation, and online influence maximization.

\subsection{Baseline Algorithms}

We compare our proposed SCUCB algorithm with both stochastic and adversarial bandits algorithms that achieves optimal asymptotic regret in their settings.
\begin{enumerate}
    \item CUCB \cite{pmlr-v28-chen13a}. CUCB is the naive counterpart of our algorithm. The algorithm calculates a upper confidence interval for each arm and pick the best arm subset with the highest upper confidence interval. 
    \item TSCB \cite{wang2018thompson}. TSCB is the combinatorial version of the classical Thompson sampling algorithm. The algorithm maintain a prior beta distribution estimation for each arm and updates according to the received reward. At each time, the algorithm samples from the estimated distributions and pick actions according to the highest sample. 
    \item Combinatorial variant of EXP3 \cite{auer_nonstochastic_2002}. The algorithm maintains a weight for each arm and draw actions according to the normalized weight distribution. Upon receiving rewards, the algorithm update weight according to the classical EXP3 update rule. 
\end{enumerate}

\subsection{Synthetic Experiments}

We conduct experiments presented in this section with synthetic data and compare our proposed algorithm with its naive counter part. The approximation oracle is designed to succeed with probability $1$. Each bandit arm is modeled to follow a Bernoulli distribution with randomly populated $\mu \in [0,1]$ and all arms adapt LSI strategy. 
The arms in the optimal arm subset have a strategic budget of $0$ since additional strategic budget for optimal arms would only boost the performance of our algorithm. All other arms are equipped with a randomly allocated budget $B$,$ 0 \leq B \leq B_{max}$ by definition. 
As is typical in the bandit literature, for example in \citet{auer2002finite}, we evaluate both the naive and strategic CUCB algorithms on their tuned versions, where the UCB exploration parameter is scaled by a constant factor $\gamma \in [0,1]$. To ensure reproducible result, each experiment is repeated for $10$ random seeds and the averaged result is presented.  

\begin{table}[H]
\centering
\label{table:1}
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{5}{c}{Cumulative regret, Action size = 2, K = 10}                                       \\ \midrule
\multicolumn{1}{l|}{Dataset}        & \multicolumn{4}{c}{Synethetic}                                        \\ \midrule
\multicolumn{1}{l|}{Bmax}           & 70              & 90              & 110             & 130             \\
\multicolumn{1}{l|}{CUCB}           & 171.74          & 187.51          & 259.04          & 256.66          \\
\multicolumn{1}{l|}{\textbf{SCUCB}} & \textbf{143.85} & \textbf{172.57} & \textbf{208.53} & \textbf{233.57} \\ \bottomrule
\end{tabular}
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{5}{c}{Cumulative regret, Action size = 2, K = 20}                                        \\ \midrule
\multicolumn{1}{l|}{Dataset}        & \multicolumn{4}{c}{Synethetic}                                         \\ \midrule
\multicolumn{1}{l|}{Bmax}           & 70              & 90              & 110             & 130              \\
\multicolumn{1}{l|}{CUCB}           & 434.82          & 492.02          & 520.97          & 549.57           \\
\multicolumn{1}{l|}{\textbf{SCUCB}} & \textbf{301.57} & \textbf{365.94} & \textbf{450.10} & \textbf{505.453} \\ \bottomrule
\end{tabular}
\caption{Cumulative regret achieved by UCB and SCUCB with synthetic data with various action size.}
\end{table}

The first set of experiment is conducted with $K = \{10, 20\}$ arms through a time horizon of $T=5000$ time steps with maximum possible budget of $B_{max} = \{70, 90, 110, 130\}$. The algorithms are asked to select $\text{Action size} = 2$ arms as an arm subset at each time step. The cumulative regret incurred by CUCB and SCUCB algorithm are presented in the table \ref{table:1} where the performance of our proposed SCUCB algorithm is highlighted in bold text. Clearly, SCUCB demonstrated its effectiveness as it achieves significantly smaller regrets in various possible maximum strategic budget. 

The next two tables reveals the advantage of SCUCB algorithm with various size of action set. The experiments are conducted with time horizon of $T=5000$ time steps with $K = \{10, 20\}$ arms and maximum possible budget of $B_{max} = \{50\}$. The algorithms are asked to select $\text{Action size} = \{2, 4, 6, 8\}$ arms as an arm subset at each time step. Once again, our SCUCB outperforms its naive counterpart by achieving much smaller cumulative regret, for which numerical results are highlighted in bold text. 
\begin{table}[H]
\centering
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{5}{c}{Cumulative regret, Bmax = 50, K = 10}                                            \\ \midrule
\multicolumn{1}{l|}{Dataset}        & \multicolumn{4}{c}{Synethetic}                                       \\ \midrule
\multicolumn{1}{l|}{Action Size}    & 2               & 4               & 6               & 8              \\
\multicolumn{1}{l|}{CUCB}           & 140.21          & 150.88          & 158.22          & 123.91         \\
\multicolumn{1}{l|}{\textbf{SCUCB}} & \textbf{105.58} & \textbf{113.63} & \textbf{103.42} & \textbf{88.72} \\ \bottomrule
\end{tabular}
\begin{tabular}{@{}lcccc@{}}
\toprule
\multicolumn{5}{c}{Cumulative regret, Bmax = 50, K = 20}                                             \\ \midrule
\multicolumn{1}{l|}{Dataset}        & \multicolumn{4}{c}{Synethetic}                                        \\ \midrule
\multicolumn{1}{l|}{Action Size}    & 2               & 4               & 6               & 8               \\
\multicolumn{1}{l|}{CUCB}           & 302.10          & 316.09          & 340.52          & 328.80          \\
\multicolumn{1}{l|}{\textbf{SCUCB}} & \textbf{232.23} & \textbf{247.32} & \textbf{268.27} & \textbf{306.77} \\ \bottomrule
\end{tabular}
\caption{Cumulative regret achieved by UCB and SCUCB with synthetic data with various $B_{max}$.}
\end{table}
%Synthetic, repeat = 10, T = 5000, arm = 10
To compare the two algorithms in details, we plot the cumulative regret incurred by algorithms against the time steps. It becomes apparent that the SCUCB algorithm features a cumulative regret versus time steps line that is much smaller than the one caused by CUCB even under a higher maximum possible strategic budget. We compare the two algorithm under settings where the maximize possible budget is $B_{max} = 70, 90$ and $B_{max} = 110, 130$.
\begin{figure}[H]
\centering
\subfigure[]{
\label{Fig1}
\includegraphics[width=3.8cm]{figs/B7090_K20_N10000.png}}
\subfigure[]{
\label{Fig2}
\includegraphics[width=3.8cm]{figs/B110130_K20_N10000.png}}
\caption{\ref{Fig1} Comparison of CUCB and SCUCB with $B_{max} = 70, 90$. \ref{Fig2} Comparison of CUCB and SCUCB with $B_{max} = 110, 130$.}
%\caption{\ref{Fig1} CUCB algorithm performance with maximize possible budget of $B_{max} = 70$ and SCUCB algorithm performance with maximize possible budget of $B_{max} = 70, 90$ \ref{Fig2} C CUCB algorithm performance with maximize possible budget of $B_{max} = 110$ and SCUCB algorithm performance with maximize possible budget of $B_{max} = 110, 130$.}
\end{figure}

\subsection{Online Worker Selection in Crowdsourcing Systems}
We simulated a online crowdsourcing system that has a workflow resembled by \ref{crowdsys} and model it as a combinatorial bandits problem. We performed extensive empirical analysis of our SCUCB algorithm against CUCB, the combinatorial version of Thompson sampling and EXP3. The experiments were conducted with the Amazon sentiment dataset, where Amazon items reviews are labeled 'is/is not book' or 'is/is not negative \cite{Krivosheev:2018:CCM:3290265.3274366}. We split the dataset into two, where 'is book' contains data that only has labels 'is/is not book' and 'is negative' contains data that only has labels 'is/is not negative'. Both dataset consists of 7803 reviews, 284 workers, and 1011 tasks. 
The correctness of workers and tasks can be visualized by the figures as below. 
\begin{figure}[H]
\centering
\subfigure[]{
\label{worker}
\includegraphics[width=3.8cm]{figs/worker_visual.png}}
\subfigure[]{
\label{task}
\includegraphics[scale = 0.28]{figs/task_visual.png}}
\caption{\ref{worker} Visualization of correctness of worker's labels. \ref{task}Visualization of correctness of task's labels.}
\end{figure}

For each task, the data contains responses from 5 workers and the crowdsourcing platform is asked to select 2, 3, or 4 workers at each time step. To measure the performance of the algorithms, we made the assumption that the reward is monotonically correlated to the accuracy of label compared to ground truth label. Thus, we define the reward to be 1, if the worker's label is the same with ground truth label and 0 otherwise. To model the strategic behavior of the workers, we model each worker with a randomly allocated strategic level $s \in [0,1]$ such that the worker provides its honest response with probability $s$. 

\begin{table}[H]
\label{first}
\centering
\begin{tabular}{@{}lccc@{}}
\toprule
\multicolumn{4}{c}{Crowdsourcing (Cumulative Reward), Bmax = 500}                            \\ \midrule
\multicolumn{1}{l|}{Dataset}        & \multicolumn{3}{c}{is\_book}                           \\ \midrule
\multicolumn{1}{l|}{Action size}    & 2                & 3                & 4                \\ \midrule
\multicolumn{1}{l|}{CUCB}           & 31672.6          & 46181.2          & 68244.6          \\
\multicolumn{1}{l|}{TSCB}          & 19853.0          & 34226.2          & 60621.2          \\
\multicolumn{1}{l|}{EXP3}           & 31569.6          & 46570.6          & 68482.2          \\
\multicolumn{1}{l|}{\textbf{SCUCB}} & \textbf{32082.6} & \textbf{46623.6} & \textbf{68524.6} \\ \bottomrule
\end{tabular}
\begin{tabular}{@{}lccc@{}}
\toprule
\multicolumn{4}{c}{Crowdsourcing (Cumulative Regret), Bmax = 500}                            \\ \midrule
\multicolumn{1}{l|}{Dataset}        & \multicolumn{3}{c}{is\_book}                           \\ \midrule
\multicolumn{1}{l|}{Action size}    & 2                & 3                & 4                \\ \midrule
\multicolumn{1}{l|}{CUCB}           & 27787.4          & 42198.8          & 48125.4          \\
\multicolumn{1}{l|}{TSCB}          & 39607.0          & 54153.8          & 55748.8          \\
\multicolumn{1}{l|}{EXP3}           & 27890.4          & 41809.4          & 47887.8          \\
\multicolumn{1}{l|}{\textbf{SCUCB}} & \textbf{27377.4} & \textbf{41756.4} & \textbf{47845.4} \\ \bottomrule
\end{tabular}
\end{table}
\begin{table}[H]\centering
\begin{tabular}{@{}lccc@{}}
\toprule
\multicolumn{4}{c}{Crowdsourcing (Cumulative Reward), Bmax = 500}                            \\ \midrule
\multicolumn{1}{l|}{Dataset}        & \multicolumn{3}{c}{is\_negative}                       \\ \midrule
\multicolumn{1}{l|}{Action size}    & 2                & 3                & 4                \\ \midrule
\multicolumn{1}{l|}{CUCB}           & 31108.8          & 44757.6          & 59424.8          \\
\multicolumn{1}{l|}{TSCB}          & 17240.6          & 32010.4          & 51109.0          \\
\multicolumn{1}{l|}{EXP3}           & 30879.0          & 44767.2          & 58207.8          \\
\multicolumn{1}{l|}{\textbf{SCUCB}} & \textbf{31759.0} & \textbf{44843.4} & \textbf{59441.4} \\ \bottomrule
\end{tabular}
\begin{tabular}{@{}lccc@{}}
\toprule
\multicolumn{4}{c}{Crowdsourcing (Cumulative Regret), Bmax = 500}                            \\ \midrule
\multicolumn{1}{l|}{Dataset}        & \multicolumn{3}{c}{is\_negative}                       \\ \midrule
\multicolumn{1}{l|}{Action size}    & 2                & 3                & 4                \\ \midrule
\multicolumn{1}{l|}{CUCB}           & 28411.2          & 43566.2          & 56465.2          \\
\multicolumn{1}{l|}{TSCB}          & 42279.4          & 56279.6          & 64781.0          \\
\multicolumn{1}{l|}{EXP3}           & 28641.0          & 43523.4          & 57682.2          \\
\multicolumn{1}{l|}{\textbf{SCUCB}} & \textbf{27761.0} & \textbf{43446.6} & \textbf{56448.6} \\ \bottomrule
\end{tabular}

\caption{Cumulative rewards and cumulative regret attained by SCUCB and baseline algorithms with various action size on isbook dataset and isnegative datase.}
\end{table}
For the first set of experiments, we choose the maximum possible strategic budget to be $B_{max} = 500$. For actions size of $2, 3, 4$. We obtain the following cumulative rewards and cumulative regret results where SCUCB's performance is highlight in bold text. To ensure reproducible results, each experiment is repeated for 5 times and the averaged result is presented. 

To further investigate the effect of maximum possible strategic budget on the performance of algorithms, we fix the size of action size to be 2 and plot the cumulative reward/cumulative regret incurred by each algorithm again $B_{max} \in [100, 700]$. Regardless of the $B_{max}$ value, our proposed SCUCB algorithm consistently outperforms other methods. For better visualization, we omit the line for combinatorial Thompson sampling due to its relatively weaker performance. 
\begin{figure}[H]
\centering
\subfigure[]{
\label{culre}
\includegraphics[width=3.8cm]{figs/culre.png}}
\subfigure[]{
\label{culreg}
\includegraphics[width=3.8cm]{figs/reg.png}}
\caption{\ref{culre} Cumulative rewards attained by algorithms with various level of $B_{max}$.  \ref{culreg} Cumulative regrets attained by algorithms with various level of $B_{max}$.  }
\end{figure}

The results of our crowdsourcing experiments reveals the robustness of our SCUCB algorithm under strategic manipulations. It also indicates the performance of adversarial and stochastic bandits algorithms under strategic manipulations. The combinatorial variant of Thompson sampling is vulnerable under manipulations, which agrees with our expectation given that the algorithm is a Bayesian algorithm in nature and is heavily relying on estimating the underlying distribution of arms. Its estimation can be easily perturbed under strategic manipulation, and thus leads to undesired performance results. It is also expected that the SCUCB algorithm far outperform its naive counterpart, CUCB algorithm. The combinatorial version of EXP3 algorithm is the most competitive algorithm with our SCUCB. As the EXP3 algorithm was originally designed for pure adversarial setting, the algorithm has some robustness under strategic manipulations. Shown in the Figure \ref{culrereg}, the combinatorial EXP3 algorithm consistently show robustness across various level of maximum possible strategic budget. However, as our SCUCB algorithm considers the maximum possible strategic budget and thus more adaptive, SCUCB far outperforms EXP3CB as $B_{max}$ increases. 

\subsection{Online Recommendation System}

Online recommendation is a classic example of combinatorial bandits in applications. We evaluated algorithms in the latest MovieLens dataset which contains 9742 movies and 100837 rating of the movies with each rating being $1 - 5$ \cite{10.1145/2827872}. We compare the algorithms based on the total values of ratings received, i.e. recommending a movie and receiving a rating of 5 is more desired than recommending a movie and receiving a rating of 1. 
\begin{figure}[H]
\centering
\includegraphics[width=7cm]{figs/arch.png}
\caption{Experiment set up of online recommendation.}
\end{figure}
As the dataset may consists of unbalanced data for each movie, we adapted collaborative filtering and $k$-means clustering into our evaluation system. We used the collaborative filtered for training and testing and instead of recommending movies, we clustered the movies by $k$-means clustering and asked bandits algorithm to choose one cluster at each time. The movie with the highest rating in the chosen cluster is recommended. The workflow of the experiment set up is summarized in above diagram. 

We performed the evaluation with various number of clusters (10, 20 or 30) and $B_{max} = 30, 50, 70$ through a time horizon of $T = 500$. The results presented below are averages over 5 runs to ensure reproducibility. From the tables below, we concludes the effectiveness of SCUCB algorithm, which performance is highlighted in bold text. 
\begin{table}[H]
\centering
\begin{tabular}{@{}lccc@{}}
\toprule
\multicolumn{4}{c}{Recsys (Cumulative Reward), T=500, 10 clusters}                          \\ \midrule
\multicolumn{1}{l|}{Dataset}       & \multicolumn{3}{c}{Movielens}                          \\ \midrule
\multicolumn{1}{l|}{Bmax}          & 30               & 50               & 70               \\ \midrule
\multicolumn{1}{l|}{UCB}           & 2297.60          & 2494.36          & 2631.02          \\
\multicolumn{1}{l|}{TS}            & 2160.14          & 2314.76          & 2468.26          \\
\multicolumn{1}{l|}{EXP3}          & 2181.11          & 2449.28          & 2430.96          \\
\multicolumn{1}{l|}{\textbf{SUCB}} & \textbf{2305.75} & \textbf{2314.76} & \textbf{2636.07} \\ \bottomrule
\end{tabular}
\begin{tabular}{@{}lccc@{}}
\toprule
\multicolumn{4}{c}{Recsys (Cumulative Reward), T=500, 20 clusters}                          \\ \midrule
\multicolumn{1}{l|}{Dataset}       & \multicolumn{3}{c}{Movielens}                          \\ \midrule
\multicolumn{1}{l|}{Bmax}          & 30               & 50               & 70               \\ \midrule
\multicolumn{1}{l|}{UCB}           & 2469.93          & 2336.92          & 2159.25          \\
\multicolumn{1}{l|}{TS}            & 2260.20          & 1850.55          & 1905.42          \\
\multicolumn{1}{l|}{EXP3}          & 2380.74          & 2317.82          & 2025.39          \\
\multicolumn{1}{l|}{\textbf{SUCB}} & \textbf{2474.69} & \textbf{2341.19} & \textbf{2177.70} \\ \bottomrule
\end{tabular}
\begin{tabular}{@{}lccc@{}}
\toprule
\multicolumn{4}{c}{Recsys (Cumulative Reward), T=500, 30 clusters}                                       \\ \midrule
\multicolumn{1}{l|}{Dataset}       & \multicolumn{3}{c}{Movielens}                          \\ \midrule
\multicolumn{1}{l|}{Bmax}          & 30               & 50               & 70               \\\midrule
\multicolumn{1}{l|}{UCB}           & 2443.57          & 2393.88          & 2472.31          \\
\multicolumn{1}{l|}{TS}            & 2132.16          & 2248.56          & 1855.14          \\
\multicolumn{1}{l|}{EXP3}          & 2368.42          & 2265.32          & 2339.49          \\
\multicolumn{1}{l|}{\textbf{SUCB}} & \textbf{2436.43} & \textbf{2397.72} & \textbf{2476.52} \\ \bottomrule
\end{tabular}
\caption{Cumulative rewards attained by algorithms with different number of clusters $10, 20, 30$ and different level of $\{B_{max} = 30, 50, 70\}$ across 500 time steps. }
\end{table}

\subsection{Online Influence Maximization}

We implemented the online influence maximization with an offline influence maximization algorithm TIM as our oracle \cite{10.1145/2588555.2593670}. TIM is one of the offline influence maximization algorithm that achieves asymptotic optimality. We perform the experiments on two datasets. One is a simulation dataset with 16 nodes and 44 edges, the other is a 100 nodes subset from Digg dataset, where each nodes represents a user from Digg website \cite{nr}. We simulate the connectivity of edges at each time step by randomly assigning each edge a connectivity probability at the start of the experiment. 

\begin{figure}[hbt!]
\centering
\subfigure[]{
\label{test_graph}
\includegraphics[width=3.6cm]{figs/test_graph.png}}
\subfigure[]{
\label{16c2}
\includegraphics[width=3.6cm]{figs/test.png}}
\caption{\ref{test_graph} Visualization of synthetic graph for evaluation. \ref{16c2} Mean rewards attained by algorithms.}
\end{figure}

Figure \ref{test_graph} visualizes the synthetic graph we created for evaluation. We then tested the algorithms over $T = 800$ time steps with action size of 2 and maximum possible strategic budget of $B_{max} = 300$. Figure \ref{16c2} show the effectiveness of algorithms by evaluating based on the averaged nodes influenced. To ensure reproducible results, we calculate the mean of nodes influence over 100 trials. For better visualization, we kept a running mean over 50 time steps to smooth the lines. 

We then investigate the effect of action size and the results are summarized in the following two tables.
\begin{table}[hbt!]
\centering
\begin{tabular}{@{}ccccc@{}}
\toprule
\multicolumn{5}{c}{OIM (Averaged Final Reward), Bmax = 200}                                   \\ \midrule
\multicolumn{1}{l|}{Dataset}        & \multicolumn{3}{c}{Synthetic, 16 nodes, 44 edges}         \\ \midrule
\multicolumn{1}{l|}{Action size}       & 2      & 4      & 6       & 8       \\ \midrule
\multicolumn{1}{c|}{CUCB}   & 5.46          & 6.54          & 10.4           & 12.5           \\
\multicolumn{1}{c|}{TSCB}  & 6.7           & 8.50           & 10.44          & 12.7           \\
\multicolumn{1}{c|}{EXP3CB} & 5.86          & 8.14          & 10.34          & 12.46          \\
\multicolumn{1}{c|}{\textbf{SCUCB}}  & \textbf{7.44} & \textbf{9.32} & \textbf{11.16} & \textbf{13.04} \\ \bottomrule
\end{tabular}
\begin{tabular}{@{}lccc@{}}
\toprule
\multicolumn{4}{c}{OIM (Averaged Final Reward), Bmax = 200}                       \\ \midrule
\multicolumn{1}{l|}{Dataset}        & \multicolumn{3}{c}{digg, 100 nodes}         \\ \midrule
\multicolumn{1}{l|}{Action size}    & 10             & 15             & 20        \\ \midrule
\multicolumn{1}{l|}{CUCB}           & 15.64          & 20.64          & 25.32           \\
\multicolumn{1}{l|}{TSCB}          & 16.30          & 21.62          & 26.08          \\
\multicolumn{1}{l|}{EXP3}           & 12.16          & 17.76          & 21.72          \\
\multicolumn{1}{l|}{\textbf{SCUCB}} & \textbf{16.56} & \textbf{22.16} & \textbf{26.14} \\ \bottomrule
\end{tabular}
\caption{Averaged final rewards attained by algorithms with synthetic and Digg dataset with action size of 2, 800 time steps and $B_{max} = 200$.}
\end{table}



\iffalse
\paragraph{Experiment setting} 

We conduct the experiments with 10 arms where each arm subset constitutes $2$ arms unless otherwise specified. The time horizon is set to be $T = 5\times 10^3$ and the approximation oracle is designed to succeed with probability $1$. Each bandit arm follows a Bernoulli distribution with randomly populated $\mu \in [0,1]$ and all arms adapt LSI except in the discussion of arm strategies. 
The arms in the optimal arm subset have a strategic budget of $0$ and all other arms are equipped with the same strategic budget, which is $B_{max}$ by definition. The setting of heterogeneous budgets is discussed in the appendix. 
As is typical in the bandit literature, for example in \citet{auer2002finite}, we evaluate both naive and strategic CUCB algorithms on their tuned versions, where the UCB exploration parameter is scaled by a constant factor $\gamma \in [0,1]$. Each experiment is repeated $10$ times and the averaged result is presented. 

\begin{figure*}[htbp]
\centering
\subfigure[]{
\label{Fig1}
\includegraphics[scale=0.3]{figs/diff_B.png}}
\subfigure[]{
\label{Fig2}
\includegraphics[scale=0.24]{figs/linearB.png}}
\subfigure[]{
\label{Fig3}
\includegraphics[scale=0.3]{figs/LSI2.png}}
\subfigure[]{
\label{Fig4}
\includegraphics[scale=0.3]{figs/50arm.png}}

\caption{\ref{Fig1} Cumulative regret v.s. time horizon under different maximum budgets; \ref{Fig2} Cumulative regret v.s. strategic budget; \ref{Fig3} Cumulative regret under the LSI strategy and random strategy; \ref{Fig4} Cumulative regret v.s. time horizon under different number of arms in each arm subset ($B_{max} = 50$).}
\end{figure*}
%Effect of tuning UCB confidence parameter
\paragraph{Cumulative regret v.s. maximum budgets} We experiment with $B_{max} \in \{0, 10, 50, 100\}$ and $\gamma = 0.2$. Figure \ref{Fig1} highlights the failure of naive CUCB as the regret grows linearly with respect to $T$. In comparison, the regret grows in a logarithmic fashion with strategic CUCB, which agrees with our theoretical finding of the $O(\log T)$ regret bound. 
%This confirms our regret analysis result in Theorem \ref{appendixA}.

\paragraph{Cumulative regret v.s strategic budget} We conduct our empirical study with and the strategic budget ranging from $1$ to $100$ under $\gamma = 0.2$. Figure \ref{Fig2} shows that the regret is linear with the largest strategic budget $B_{max}$ under both strategic CUCB and naive CUCB, which agrees with our linear term on the budget in Theorem \ref{appendixA}. 
%This attests to our theoretical bound of regret being $O(B_{max})$ under strategic CUCB. 
We observe that, though at a small value of $B_{max}$ CUCB display unstable performance, strategic CUCB can achieve much lower regret than that of naive CUCB in general. We, therefore, conclude the superiority of strategic CUCB in small-budget and large-budget regimes.

\paragraph{Cumulative regret under LSI strategy and random strategy} We simulate the random strategy for arms as arms randomly spend a budget that is generated from a standard uniform distribution in each round. 
%We stimulate the random strategy for arms, where the arms randomly spend part of its strategic budget in probability, simulated by uniform random seed, each time the arm is pulled. 
It is illustrated in Figure \ref{Fig3} that regardless of the choice of the bandit learning algorithm, the regret under LSI is higher than the regret under a random strategy. As is discussed previously, LSI strategy is one of the most powerful strategies that strategic arms can perform to hamper regret. The effect of strategies with collusion is demonstrated in the appendix. 

\paragraph{Cumulative regret v.s. different arm subset size} We relax the number of arms in each arm subset from $2$ to $4$ and $6$ to observe the sensitivity with respect to this parameter. We choose naive CUCB with $4$ arms in each arm subset as a baseline and the maximum budget is set to be $50$. As shown in Figure \ref{Fig4}, our algorithm outperforms naive CUCB regardless of the number of arms in each arm subset, which indicates the robustness of strategic CUCB on the arm subset size.

\fi

==> strategic combinatorial WSDM/WSDM/formulation.tex <==
We consider the problem of combinatorial multi-armed bandits (CMAB) under the setting of strategic arms. In strategic CMAB, each arm is given a budget and the arm can strategically increase its emitted reward signals cumulatively up to this budget \emph{for its own interest}. This problem is a Stackelberg game which involves two parties. The bandit learning algorithm is deployed first to maximize its cumulative reward under the best response of the followers. The $m$ strategic bandits arms then deplete their budget where each of them aims to maximize its expected number of pulls. Knowing the principal's strategy and other followers' budget information, the followers are assumed to place their strategies according to the dominant Nash equilibrium between them. 

Formally, given a time horizon $T$, the the bandit learning algorithm is asked to pull a subset of arms, denoted by an arm subset $S_t \in \mathcal{S} $ at each time $t\in [T]$, where $\mathcal{S} = { \{0,1\}^{m}} $ is the set of all possible arm subsets. At time $t$, based on the principal's choice of arm subset, stochastic rewards $x_{i,t}$ are generated by arm $i$ from the underlying $1$-sub-Gaussian distribution with mean $\mu_i$, independent of other arms in $S_t$. The principal does not observe these rewards. Instead, each arm can increase the emitted reward signal by an arbitrary amount $z_{i,t}\ge 0$, as long as the cumulative manipulation over the horizon does not exceed a given budget $B_i$. The principal then receives the semi-bandit feedback $\{x_{i,t}+z_{i,t}\}_{i\in S_t}$.

%The reward of playing arm subset $S$ at time $t$ is decided by a stochastic reward function $R_t(S)$, which is a function of $\{x_{i,t}\}_{i\in S}$. 
Let $\bm{\mu} = (\mu_1, \mu_2, ..., \mu_i) $ be the vector of expectations of all arms. The expected reward of playing any arm subset S in
any round $r_{\bm{\mu}}(S) = \mathbb{E}[R_t(S)]$,which is a function of arm subset $S$ and $\bm{\mu}$. The reward function $r_{\bm{\mu}}(S)$ is assumed to satisfy two axioms:
\begin{itemize}
    \item \textbf{Monotonicity.} The expected reward of playing any arm subset $S \in \mathcal{S}$ is monotonically non-decreasing with respect to the expected reward vector. That is, if for all $i \in [m], \mu_i \leq \mu_{i}'$, then $r_{\bm{\mu}}(S) \leq r_{\bm{\mu}'}(S)$.
    \item \textbf{Bounded smoothness.} There exists a strictly increasing function $f(\cdot)$, termed the bounded smoothness function, such that for any two expected reward vectors $\bm{\mu}$ and $\bm{\mu'}$ satisfying $\|\bm{\mu}-\bm{\mu'}\|_{\infty}\le \Lambda $, we have $|r_{\bm{\mu}} - r_{\bm{\mu'}}| \leq f({\Lambda})$.
\end{itemize}
These axioms cover a rich set of reward functions and the explicit forms of $R_t(S)$ and $r_{\bm{\mu}}(S)$ are not needed to be specified \citep{pmlr-v28-chen13a}.

Without loss of generality, assume that $S^\ast = \argmax_{S\subseteq \mathcal{S}} r_{\bm{\mu}}(S)$ is the unique optimal subset of arms. When placing reward manipulations, each strategic arm has access to its own history $h_{i,t} = \{I_{i,t'}, x_{i,t'}, z_{i,t'}\}_{t'\ge 1}$, where $I_{i,t'}$ is the indicator of whether arm $i$ is pulled at time $t'$ and $t' < t$. The strategy of arm $i$ is determined by a function that maps this history to a manipulation $z_{i,t}$, as $Z_{i,t} \colon h_{i,t-1} \to \mathbb{R}$. Without loss of generality, we assume that arms in the optimal arm subset $i\in S^\ast$ have strategic budgets of $0$, which restricts their $z_{i,t}$ to be $0$.

In the combinatorial setting, even with the exact reward vector $\bm\mu$ provided, it can be hard to exactly compute the optimized $r_{\bm{\mu}}(S)$. In view of this, many have studied probabilistic approximation algorithms in combinatorial problems, which indicates that an ($\alpha,\beta$)-approximation oracle defined below can be usually available. 

\begin{definition}[Approximation oracle]
Let $0\le \alpha,\beta \leq 1$ and define ${OPT}_{\bm{\mu}} = \max_{S\in \mathcal{S}} r_{\bm{\mu}}(S)$. 
An oracle is called an ($\alpha,\beta$)-approximation oracle if it takes an expected reward vector $\bm{\mu}$ as input and outputs an arm subset $S \in \mathcal{S}$ such that $\mathbb{P}(r_{\bm{\mu}}(S) \geq \alpha \cdot {OPT}_{\bm{\mu}}) \geq \beta$. That is, the oracle gives an arm subset $S$ that is at least as good as $\alpha$ times the reward of an optimal arm subset with probability at least $\beta$. 
\end{definition}
Denote ${S_B} = \{ r_{\bm{\mu}}(S) < \alpha \cdot {OPT}_{\bm{\mu}} | S \in \mathcal{S}\}$ to be the set of suboptimal arm subsets under the approximation oracle. 
Note that a suboptimal arm subset can be given by the oracle for two reasons. The ($\alpha,\beta$)-approximation oracle can fail, which happens with probability at most $1-\beta$. The estimation of $\bm{\mu}$ can deviate from the true value by a significant amount, resulting in accurate input to the oracle.

The objective of the principal is to maximize the expected cumulative reward before manipulation over the time horizon $T$. Equivalently, the principal minimizes the regret, the cumulative difference between the scaled optimal reward and expected actual reward, as defined below. 

\begin{definition}[Regret]
With access to an ($\alpha,\beta$)-\textit{approximation oracle}, the regret of a combinatorial bandit algorithm for $T$ rounds is
\[
Regret_{\bm{\mu},\alpha,\beta}(T) = T \cdot \alpha \cdot \beta \cdot {OPT}_{\bm{\mu}} - \mathbb{E}\big[\sum^T_{t=1}r_{\bm{\mu}}(S_t)\big]\,,
\]
where the randomness in $\mathbb{E}[\sum^T_{t=1}r_{\bm{\mu}}(S_t)]$ involves the stochasticity of the bandit algorithm and the oracle.
\end{definition}

The objective of each strategic arm $i\in [m]\setminus S^{\ast}$, however, is to maximize the number $\sum_{t=1}^T I_{i,t}$ of times it is pulled over the time horizon. To achieve this, the arm needs to confuse the principal by deviating the emitted reward signals up to the possessed budget. % For a fixed bandit algorithm of the principal, the budget deployment strategies of the arms are assumed to follow the dominant Nash equilibrium $NE$. With the principal, this Stackelberg game writes
\iffalse
\begin{equation*}
\begin{aligned}
& \underset{S_t}{\mathrm{maximize}}
& & Regret_{\bm{\mu},\alpha,\beta}(T) \\
& \mathrm{subject}\text{ }\mathrm{to}
& & z_{i,t} = \argmax_{NE} \sum_{t=1}^T I_{i,t}, \ \text{for}\ t\in [T],\ i\in [m]\setminus S^*\,, \\
& & & \sum_{t=1}^T z_{i,t} \le B_i \ \text{for}\  i\in [m]\setminus S^*\,.
\label{eqn:stackelberg}
\end{aligned}
\end{equation*}
\fi

Our goal is to analyze the robustness of existing CMAB algorithms under the strategic setting and propose strategic variants that guarantee better performance.


==> strategic combinatorial WSDM/WSDM/intro.tex <==
Sequential learning methods  feature prominently in a range of real applications such as online recommendation systems, crowdsourcing systems, and online influence maximization problems. Among those methods, the multi-armed bandits problem serves as a fundamental framework. Its simple yet powerful model characterizes the dilemma of exploration and exploitation which is critical to the understanding of online sequential learning problems and their applications to real applications \citep{10.2307/2332286, Robbins:1952,auer2002finite,lattimore_szepesvari_2020}.
The model describes an iterative game constituted by a bandit algorithm and many arms. The bandit algorithm is required to, through a horizon $T$, choose an arm to pull at each time step. As the objective is to maximize the cumulative reward over time, the algorithm balances between exploiting immediate rewards based on the information collected or pulling less explored arms to gain more information about arms \citep{anantharam_asymptotically_1987,auer_nonstochastic_2002,cesa-bianchi_prediction_2006}. % One of the motivating examples to showcase the natural adaptation of MAB to real applications can be recommender systems. The bandits arms may refer to items to be recommended and the bandit algorithm, the recommender system, seek to maximize the cumulative rewards which can be measured through a range of metric. In the simplest case, the rewards can be measured through the number of clicks given by the users and a higher rate of clicking would deem beneficial to the system. 

%Many real applications involve bandit algorithms in their decision systems, including recommendation systems, medical trials, network routing, crowdsourcing systems, combinatorial optimization, automated machine learning, etc.

Out of the real applications, many motivate the extension of MAB towards combinatorial multi-armed bandits (CMAB), where multiple arms can be selected in each round \citep{pmlr-v28-chen13a,DBLP:conf/nips/CombesSPL15,pmlr-v48-lif16,pmlr-v97-zimmert19a,pmlr-v117-rejwan20a}. CMAB demonstrates its effectiveness on problems like online social influence maximization, viral marketing, and advertisement placement, within which many's offline variants are NP-hard. However, existing MAB and CMAB algorithms are often developed either under benign assumptions on the arms \citep{pmlr-v28-chen13a,pmlr-v38-kveton15,pmlr-v75-wei18a} or purely adversarial arms \citep{auer2002nonstochastic}. In the former setting, the arms are commonly assumed to report their reward signals truthfully without any strategic behavior, under which the drawbacks are apparent.

In the later setting, arms can attack any deployed algorithm to a regret of $O(T)$ with this capability of reward manipulations, which is catastrophic for a bandit algorithm. 
This assumption is stringent and rarely realistic.

In this paper, we first rigorously analyze the difference between the assumptions placed on the adaptive arms and the regret upper and budget lower bounds thereof, in both MAB and CMAB. 
These justify our intuition that strategic manipulation is indeed a weaker assumption on arms' influence on the regret.
To put forward a bandit algorithm under strategic arms, we adapt the combinatorial UCB (CUCB) algorithm with a carefully designed UCB-based exploration term. 
A major difficulty stems from not knowing the manipulation term made by the arms, while our algorithm overcomes this by depending only on the knowledge of the maximum possible strategic budget.
New tail bounds over the proposed exploration term and a new trade-off parameter that balances exploration and exploitation are utilized to facilitate the analysis of our algorithm.
We further establish results on the robustness of our UCB variant under strategic arms with an algorithm-dependent budget lower bound.

Our proposed algorithms are also evaluated empirically through an extensive set of synthetic environments and real datasets. 
The real applications include reliable workers selection in online crowdsourcing systems, where workers might misrepresent a result for a better chance to be selected in the future; online information maximization, where nodes modify the spread to include itself into the seed set; and online recommendation systems, which characterizes the ``click framing'' behavior. Through a wide range of tasks and parameters, the experiment results corroborate our theoretical findings and demonstrate the effectiveness of our algorithms.

\subsection{Motivating Examples}
\input{motivation}



==> strategic combinatorial WSDM/WSDM/lower.tex <==
To fully understand the effects of strategic manipulations, we investigate the relationship between the strategic budget and the performance of UCB-based algorithms. Our results provide the dependency between an arm's strategic budget and the number of times it is pulled, which influence the regret of the algorithm incurred by the arm. Our analysis gains some insight from \citet{zuo_near_2020}, which limits the discussion to the 2-armed bandit setting and cannot be applied to the general MAB setting directly. 

%Counter-intuitively, the dependency between the number of pulls of a strategic arm and its strategic budget is linear and subsequently, this infers that the regret depends on each strategic budget linearly.
%For a strategic arm to manipulate the algorithm to suffer an undesired regret of $\omega(k)$, where $k\ge O(\log T)$, the strategic budget must be at least $\omega(k)$.
%We formalize this statement in Theorem \ref{lower}, while we defer the complete proof to the appendix.

We first define some notations used in the theorem.
Without loss of generality, let arm $i^{\ast}$ be the optimal arm and arm $i, i \neq i^{\ast}$ be an arbitrary strategic suboptimal arm. Assume that arm $i$ has no access to the information regarding other arms. Let $K_{i,t}$ and $K_{i^{\ast},t}$ denote the number of times arm $i$ and arm $i^{\ast}$ have been pulled up to time $t$, respectively. Denote $\hat{\mu}_{i,t}$ as the empirical estimate of the underlying mean $\mu$ without manipulations, i.e., $\hat{\mu}_{i,t} = \frac{\sum^{t-1}_{j=1}x_{i,j}}{K_{i,t-1}}$. Define the suboptimality gap for each strategic arm $i$ to be $\delta_i = \mu_{i^{\ast}} - \mu_i$. We use a slightly revised UCB algorithm as the basic algorithm, where the UCB estimation term for arm $i$ is $\hat{\mu}_{i,t} + \sqrt{\frac{2\log(K_{i,t}^2/\eta^2)}{K_{i,t}}}$ and $\eta$ is a confidence parameter chosen by the algorithm.

\begin{theorem}\label{lower}
In stochastic multi-armed bandit problems, for a strategic suboptimal arm $i$ without access to other arms' information, to be pulled for $\omega(k)$ in $T$ steps under the UCB algorithm where $k\ge O(\log{T})$, the minimum strategic budget is $\omega(k)$. 
%The regret incurred is thus $\omega(\log{T})$. 
\end{theorem}

\iffalse
\begin{proof}[Proof sketch] 
Let $t \in [1,T]$ be the time step arm $i$ is pulled for the last time, the following inequality must stand
\begin{align*}
& \hat{\mu}_{i,t} + \sqrt{\frac{2\log(K_{i,t}^2/\eta^2)}{K_{i,t}}} + \frac{\rho_i}{K_{i,t}}\geq \hat{\mu}_{i^{\ast},t} + \sqrt{\frac{2\log(K_{i^{\ast},t}^2/\eta^2)}{K_{i^{\ast},t}}}\,.
\end{align*}
By the Chernoff-Hoeffding bound and the union bound, 
\begin{align*}
\quad \mathbb{P} \left(\hat{\mu}_{i,t}  - \mu_i  \geq \sqrt{\frac{2\log(K_{i,t}^2/\eta^2)}{K_{i,t}}}\right) \leq  \frac{\pi^2}{6} \eta^2 \,.
\end{align*} 
Hence, with probability $1 - 2 \frac{\pi^2}{6}\eta^2$, we have %$(1 - \eta^2 \frac{\pi^2}{6})^2$, 
\begin{align}
\mu_i + \sqrt{\frac{2\log(K_{i,t}^2/\eta^2)}{K_{i,t}}} + \frac{\rho_i}{K_{i,t}} \geq \mu_{i^{\ast}}\,. \notag
\end{align}
When arm $i$ is pulled, arm $i$ wants to ensure the following holds
\begin{align}
 \sqrt{\frac{2\log(K_{i,t}^2/\eta^2)}{K_{i,t}}} + \frac{\rho_i}{K_{i,t}} \geq \delta_i\,,\notag
\end{align}
where $\delta_i = \mu_{i^{\ast}} - \mu_i$. Then,
\begin{equation*}
B_i \geq \rho_i \geq \left(\delta_i - \sqrt{\frac{2\log(K_{i,t}^2/\eta^2)}{K_{i,t}}}\right) \cdot K_{i,t}\,.  \qedhere
\end{equation*}
\end{proof}
\fi 
This dependency of $k$ can be extended to CMAB and CUCB straightforwardly when arms within an arm subset collude. Counter-intuitively, the dependency between the number of pulls of a strategic arm and its strategic budget is linear and subsequently, this infers that for a strategic arm to manipulate the algorithm to suffer an undesired regret of $\omega(k)$, where $k\ge O(\log T)$, the strategic budget must be at least $\omega(k)$.

==> strategic combinatorial WSDM/WSDM/motivation.tex <==
The setting of strategic manipulations describes the strategic behavior found in a variety of real applications. We discuss two popular applications in details, namely workers selection in online crowdsourcing platforms and online influence maximization through social networks. 

\subsection{Online Worker Selection in Crowdsourcing Platforms}

Consider a crowdsourcing platform that provides data labelling service for a payment. The platform interact with a group of customers and a pool of workers. The customers request tasks to the platform for labeling and the platform is then responsible of selecting workers from the worker pool to complete the tasks. This process repeats, during which the platform learns the best deployment. We maintain a mild assumption that the payments from customers are non-decreasing with the quality of labels. To maximize its profit, it is desired for the platform to select workers that provides most reliable labels. The workflow of the platform can be described in the diagram below. %\ref{crowdsys}. 

While the platform and the customers desire quality labels, it may not entirely be in the worker's interest to exert highest effort and thus report quality labels each time, which factors into a range of reasons. Workers may adapt strategic behaviors to maximum their own utility instead. Thus, it becomes crucial to identify the reliable workers to prevent strategic behaviors that jeopardize profits.
This naturally translate to a combinatorial multi-armed bandits problem under strategic manipulations where the workers are the strategic arm and the payments acts as the rewards.

\begin{figure}[H]
\centering
\label{crowdsys}
\includegraphics[width=7.5cm]{figs/crowdsys.png}
\caption{Online crowdsourcing system}
\end{figure}

\subsection{Online Influence Maximization}

For a social network that can be represented by the below directed graph where white dots are people and black dots labeled with ``SI'' are social influencers. The temporal nature of social network results in each directed edges exists with a probability at each time step. Formally, a node is said to be reached by a seed node if there it has a directed path from the seed node. Note that this definition considers a diffusion process where a node can be reached by a seed node through multiple edges. Given a set of seed nodes, we define a spread across social network at a given time $t$ by the expected number of nodes that can be reached by the nodes in the seed node set at that time. Intuitively, this models information spread among social networks and reflects scenarios like viral marketing.

\begin{figure}[H]
\centering
\includegraphics[scale = 0.35]{figs/example.png}
\caption{Probabilistic social network}
\end{figure}

In the case of product marketing, a company may need to select the most influential social influencers to collaborate with to maximize the expected spread across time. This can be expressed as an online influence maximization problem as the company seek to maximize the size of population reached by promotions across number of promotions. However, in many cases social influencers may report inaccurate information regarding their social influential ability, which may corresponds to a number of ways in real applications, such as faking follower numbers on social media platforms. 


==> strategic combinatorial WSDM/WSDM/related.tex <==

\iffalse
\begin{table*}[t]
\begin{tabular}{|c|c|c|c|c|}
\hline
\multicolumn{5}{|c|}{Problem Formulation}                                                                             \\ \hline
\multicolumn{1}{|l|}{}                                        
& \begin{tabular}[c]{@{}c@{}}Pure\\ Adversarial\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}Adversarial \\ Attack\end{tabular}                                  
& \begin{tabular}[c]{@{}c@{}}Adversarial \\ Corruption\end{tabular}                                  
& \begin{tabular}[c]{@{}c@{}}Strategic\\ Manipulations\end{tabular}                                                     \\ \hline
\begin{tabular}[c]{@{}c@{}}Budget \\ constraints\end{tabular} & None                                                  & \begin{tabular}[c]{@{}c@{}}Group\\ constraints\end{tabular}                                    
& \begin{tabular}[c]{@{}c@{}}Group\\ constraints\end{tabular}                                        
& \begin{tabular}[c]{@{}c@{}}Individual\\ constraints\end{tabular}                                                    \\ \hline
Objective                                                     
& Unspecified                                                
& \begin{tabular}[c]{@{}c@{}}Group\\ interest\end{tabular}                                       
& \begin{tabular}[c]{@{}c@{}}Group\\ interest\end{tabular}                                           
& \begin{tabular}[c]{@{}c@{}}Individual \\ interest\end{tabular}                                                      \\ \hline
Regret        
& $O(\sqrt{T})$  \citep{NIPS2014_25b2822c}
& \begin{tabular}[c]{@{}c@{}}Attack cost of $O(\log T)$ \\ with $\omega(T)$ regret \\ \citep{NEURIPS2018_85f007f8}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}Identify best arm with up to\\  $O(\sqrt{T/K})$ corruption \\ \citep{pmlr-v99-gupta19a}\end{tabular} 
& \begin{tabular}[c]{@{}c@{}}$O(\log T)$  \\ \citep{pmlr-v119-feng20c}\end{tabular} \\ \hline
\end{tabular}
\caption{\label{tab:summary}Summary of various bandit problems.}
\end{table*}
\fi

The problem of multi-armed bandits (MAB) was first investigated back to 1952 while some techniques utilized was developed back to 1933 \citep{10.2307/2332286, Robbins:1952, berry,auer2002finite,lattimore_szepesvari_2020}. Since then it has been extensively explored and serves as the foundation of many modern areas, including reinforcement learning, recommendation systems, graph algorithms, etc. \citep{DBLP:conf/iconip/BouneffoufBG12,pmlr-v70-vaswani17a, pmlr-v85-durand18a, li2020stochastic}. With the need to model the selection of multiple arms in one round, MAB is then extended to combinatorial multi-armed bandits (CMAB), %The latter, despite being more complicated to analyze and implement, covers a richer set of settings and has a better synergy with offline approximation algorithms who can be used as oracles. CMAB algorithms 
which see many deployments in real applications like news/goods recommendation, medical trials, routing, and so forth \citep{Wang_Ouyang_Wang_Chen_Asamov_Chang_2017,8022964,pmlr-v84-sankararaman18a, li2020online}. 

%Though many studies focus on stochastic MAB and stochastic CMAB, which are the vanilla settings that the rewards of arms are independent and drawn from stationary distributions, 
Real applications motivate the community to derive algorithms in more adaptive environments.% compare to the vanilla settings that the rewards of arms are independent and drawn from stationary distributions. 
The first of which considers adversarial bandits with the classic EXP3 algorithm. The arms are assumed to be non-stationary but non-adaptive (which means that algorithms will adapt to the adversarial) \cite{auer2002nonstochastic}. Despite that adversarial bandits do not fall under the scale of this paper's related work, it leads tremendous effort to the following topics in adaptive arms.% and it is technically the Lagrangian dual of bandits with adversarial corruptions.

\paragraph{Adversarial corruptions}
%Adversarial corruption in bandits is a form of adaptive reward that poses relatively the largest difficulty for bandit algorithms. 
The adversary is given the ability to replace the observations of the bandit algorithm with arbitrary values within some constraints.
\citet{pmlr-v99-gupta19a} discuss the constraint that rewards are modified for at most $T_0$ rounds out of the total $T$ rounds. The asymptotic regret bound $O(mT_0)$ achieved in the work is shown to match the negative result, where $m$ is the number of arms. \citet{lykouris_stochastic_2018} discussed a different constraint where the corruption $z_t$ at time $t$ is cumulative up to some constant $B$%, which writes $\sum^T_{t=1} z_t \leq B$. 
The regret achieved under this constrained corruption is bounded by $O(mB\log(\frac{mT}{\delta}))$ with probability at least $1 - \delta$. \citet{JMLR:v20:18-395} restricts corruptions as independent Bernoulli events with probability $b$, while if corruption happens the reward becomes arbitrary and adversarial. This problem is addressed with median statistics with gap-dependent matching regret upper and lower bounds of $O(\sum_{i \neq i^{\ast}} \frac{1}{\Delta_i}\log(\frac{K}{\Delta_i}))$, where $i^{\ast}$ denotes the optimal arm and $\Delta_i$ is the suboptimality of arm $i$.

Several lines of research also discuss corruption topics in frequentist inference and partial monitoring \citep{pmlr-v83-gajane18a}, best arm identification \citep{pmlr-v99-gupta19a}, and adversarial bandits \citep{NEURIPS2020_e655c771}.

\paragraph{Adversarial attacks}
Different from arms in adversarial corruptions who intend to maximize the regret of the bandit algorithm, arms in the adversarial attack setting have the goal to maximize their number of pulls. 
%The objectives of the bandit algorithm and the arms do not agree in general, but they are not completely opposite either. 
The setting is first considered by \citet{NEURIPS2018_85f007f8}, where it shows that the attacker may spend a budget of $O(\log T)$ to deceit UCB and $\epsilon$-greedy algorithms to pull the target arms for at least $T - o(T)$ times. Stochastic and contextual MAB algorithms also suffer from undesired loss from this adversarial attack, under a variety of attack strategies \citep{pmlr-v97-liu19e}. Linear MAB algorithms, however, are shown to be near-optimal up to some linear or quadratic terms on the attack budget $B$ \citep{garcelon_adversarial_2020,bogunovic_stochastic_2020}. 

\paragraph{Strategic manipulations}
The setting of strategic manipulations further weakens the capability of the adaptive arms and prevents the bandit algorithms from being overcautious. 
The objective of an arm is still utility maximization under strategic manipulations, while each arm works on its utility individually. 
Instead of having a global coordinator for the adversarial attack strategy, the strategic arms seek the best response via the dominant Nash equilibrium. 
The strategic manipulation setting is first studied by \citet{pmlr-v99-braverman19b} where each arm is assumed to keep portion of the reward in each round and arms maximize the cumulative reward it keeps. 
The performance of bandit algorithms will then be catastrophic under the dominant Nash equilibrium, receiving an expected cumulative reward of $0$ almost surely. 
With the utility of maximizing the number of pulls for each strategic arm, common bandits algorithms are proved to be robust with guaranteed $O(\log T)$ regret bound, but only under constant strategic budgets \citep{pmlr-v119-feng20c}. 
For $\omega(\log T)$ budgets, bandits under strategic manipulations remain an open problem and will be discussed in this paper. 

%\citet{pmlr-v119-feng20c} is the first to study regret minimization under the strategic bandit setting. The work investigated various classical bandit algorithms, such as UCB, $\epsilon$-greedy and Thompson Sampling, and certify the robustness of these algorithms with a regret of $O(\log T)$. However, the lower bound presented in the work is logarithmic dependent and become vacuous when B is of $O(\log T)$


==> strategic combinatorial WSDM/WSDM/strategy.tex <==
%There exists a range of assumptions on the underlying stochastic game in the multi-armed bandit frameworks. On one extreme of the spectrum is the adversarial bandit problem, where the algorithm observes rewards that are presumed to be chosen by an adversary. On the other extreme, we have the stochastic bandit problem where the observed rewards generated by each arm are associated with a stationary distribution. Most real applications, however, fall somewhere on this spectrum in between the extreme points. Previous works on bandit problems with adversarial attack \citep{NEURIPS2018_85f007f8,pmlr-v97-liu19e,garcelon_adversarial_2020,bogunovic_stochastic_2020}, adversarial reward corruptions \citep{lykouris_stochastic_2018,pmlr-v99-gupta19a,JMLR:v20:18-395}, and strategic manipulations \citep{pmlr-v99-braverman19b,pmlr-v119-feng20c} aim to give the most suitable descriptions of the real problems. 

From a game-theoretical point of view, %the optimal collusion strategy of bandit arms serves as a bridge towards different acknowledgments of arms' individual interests. 
by considering collusion, we can reduce the underlying bi-levels stochastic game in bandits with strategic manipulations to a two-party game with the learning algorithm and the arms and thus have a standard to gauge the performance of algorithms along with the hardness of each bandit problems. This positions the setting of strategic manipulations among existing settings like adversarial corruptions and adversarial attacks.

%We start by discussing the optimality of the lump sum investing (LSI) strategy, the subgame perfect dominant strategy, under collusion. 
%Despite that \citet{pmlr-v119-feng20c} prove the subgame dominance among arms of lump sum investing (LSI) strategy, 
We present a counter-example where the subgame dominant strategy the lump sum investing (LSI) strategy is suboptimal when the arms collude \citet{pmlr-v119-feng20c}. % under the common goal of regret maximization. 
Consider a three arms bandit instance with mean $\mu, \mu - \Delta, \mu - 2\Delta$ expected rewards, respectively. 
With the UCB algorithm, the first three time steps are for initialization where the algorithm pulls each arm once. 
%Clearly, any strategy is an optimal collusion strategy for the time horizon of $T = 1, 2, 3$. 
When the time horizon $T$ is $4$, however, the optimal strategy would lure the algorithm to pick arm 3 at time step 4. 
This objective is achieved when arm 3 spends all of its strategic budgets whenever it is first pulled and lets arm 2 be truthful about its emitted rewards. 
Under the LSI strategy, both arm 2 and arm 3 would spend all of their strategic budgets when they are first pulled, which happens in the initialization rounds.
%When the time horizon $T=5$, the optimal collusion strategy becomes letting arm 3 spends all of its budgets when it is first pulled, letting arm 2 spends $\Delta$ when it is first pulled, and spends the rest of its budget on its second pull. Under this strategy, arm 3 is guaranteed to be pulled at time step 4 if it possesses enough strategic budgets to alter rewards higher than the optimal arm is capable of. As arm 2 spends $\Delta$, which is exactly the suboptimality gap, arm 2 is just as good as the optimal arm at a time step of 5. 

We then establish a portrayal of the optimal collusion strategy by formulating the problem into a combinatorial optimization problem. % under the goal of maximizing the number of suboptimal pulls. 
%It is a similar formulation with the regret maximization problem our counter-example is built on, which will be deferred to the appendix. 
%Extensive empirical results on the optimality of variants of LSI as collusion strategies are also discussed in the appendix.
%but under the objective of maximizing regret along with 

%\subsection{Suboptimal pulls maximization}
\begin{claim}
Under a strategic stochastic multi-armed bandit problem, when the strategic suboptimal arms collude to maximize the number of suboptimal pulls of the UCB algorithm with confidence parameter $\sqrt{\frac{3\log t_i}{K_{i,t-1}}}$, the maximum number of suboptimal pulls is the solution of 
\begin{equation*}
\begin{aligned}
& \underset{Y_{i},t_i,\ i\in [m]}{\mathrm{maximize}}
& & Y_{1}+\dots+Y_{m} \\
& \mathrm{subject}\text{ }\mathrm{to}
& & \frac{B_i}{Y_{i}} + \sqrt{\frac{3\log t_i}{Y_{i}}} \ge \delta_i + \sqrt{3\log t_i},\ i \in [m]\,, \\
& & &  t_{i_j} \ge \sum_{l=1}^j Y_{i_l}, \ j\in [m]\,,\\
& & &  \textup{for some permutation}\ i_1,\dots\ i_m\ \textup{of}\ [m]\,.\\
\end{aligned}
\end{equation*}
%\begin{align*}
%&\textup{maximum} \ K_{1,T}+\dots+K_{m,T}\\
%& \textup{subject to} \ \ \frac{B_i}{K_{i,t-1}} + \sqrt{\frac{3\log t_i}{K_{i^,t-1}}} \ge \delta_i + \sqrt{3\log t_i},\ i \in [m] \\
%&\text{there exists a permutation}\ \ i_1, \dots, i_{m-1}\\
%&t_{i_1} \ge K_{i_1}\\
%&t_{i_2} \ge K_{i_1} + K_{i_2}\\
%&\dots \\
%&t_{i_{m-1}} \ge K_{i_1} + \dots + K_{i_{m-1}}\\
%\end{align*}
\end{claim}
In the program, $Y_i$ represents the total number of times arm $i$ is pulled, which corresponds to $K_{i,T-1}$ used in previous sections. The permutation $i_1,...,i_m$ then describes, before the optimal arm is first pulled, the chronological order of the suboptimal arms to complete their last pull.
Observe that the confidence parameter of the optimal arm %$\frac{B_i}{K_{i,t-1}} + \sqrt{\frac{3\log{t}}{K_{i,t-1}}} - \sqrt{\frac{3\log{t}}{K_{i^{\ast},t-1}}}$ 
increases with respect to $t$, the inequality holds for $t_i$ if and only if it holds for all $t\le t_i$.
%With the constraint that the total number of pulls must not exceed the time index.%, we obtain the complete combinatorial program.
%The above-mentioned assumption is natural for the optimal strategy under collusion. Intuitively, two suboptimal arms should not be `competing' to get pulled. In other words, the optimal strategy ensures that the inequality stands for one suboptimal arm $i \in [m]$ uniquely. The optimal strategy search for a permutation $i_1,...,i_m$, which $i_j$ describes the last time where a strategic arm $j$ is pulled.
%Under the UCB algorithm, a suboptimal arm $i, i \neq i^{\ast}$ is pulled if and only if the following inequality stands
%\begin{align*}
%     \frac{B_i}{K_{i,t-1}} + \sqrt{\frac{3\log(t)}{K_{i,t-1}}} \geq \delta_i + \sqrt{\frac{3\log(t)}{K_{i^{\ast},t-1}}}\,.
%\end{align*}
%Hence the search for optimal collusion strategy is equivalent to the search for a combination of arms spending budgets to optimize the number of times the inequality holds. As $K_{1,T}+\dots+K_{m,T}$ records the number of times this inequality is true, the combinatorial optimization objective can be written in terms of maximizing $K_{1,T}+\dots+K_{m,T}$.
By the same observation that the advantage of the optimal arm increases with time, %it is, therefore, in a bandit arm's best interest to spend its strategic budget as early as possible. 
%Based on this observation, 
strategic arms who optimally spend their budgets for the maximum amount of pulls will also maximize their number of pulls till the first optimal arm pull. 
The inequality condition of the combinatorial program is thus $\frac{B_i}{K_{i,t-1}} + \sqrt{\frac{3\log t_i}{K_{i,t-1}}} \ge \delta_i + \sqrt{3\log t_i}$. 
We term the class of approximately optimal strategy as `sequential pull strategy', in which the strategic arms deceit the learning algorithm to pull suboptimal arms until the depletion of the budgets and this class includes the LSI strategy.

%The inequality $\frac{B_i}{K_{i,t-1}} + \sqrt{\frac{3\log t}{K_{i,t-1}}} \ge \delta_i + \sqrt{\frac{3\log t}{K_{i^{\ast},t-1}}}$ is a necessity for arm $i$ to be pulled, and will be sufficient under the assumptions that no suboptimal arms compete for the pulls. This condition translates to the case where the inequality does not simultaneously hold for two suboptimal arms. We conjecture that the condition must hold for some optimal strategy by carefully designing the initial budget commitments. When the condition holds, the inequality term $t_{i_j} \ge \sum_{l=1}^j Y_{i_l}$ can then be relaxed to an equality $t_{i_j} = \sum_{l=1}^j Y_{i_l}$.

%Knowing this, we build the intuition that the search for optimal collusion strategy lay on the search of optimal order of budget spending, in accordance to some priorities dependent of arm's background information and optimization objective.

==> strategic combinatorial WSDM/util.tex <==
\usepackage{amsmath}
\usepackage{sansmath}
\usepackage{bm}
\usepackage{float}
\usepackage{graphicx}
\usepackage{float} 
\usepackage{subfigure}
\usepackage{amsfonts}
\usepackage{amsthm}
%\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{xcolor}
\usepackage{stfloats}
\usepackage{lipsum}
\usepackage{fullpage}
\makeatletter
\newtheorem*{rep@theorem}{\rep@title}
\newcommand{\newreptheorem}[2]{%
\newenvironment{rep#1}[1]{%
 \def\rep@title{#2 \ref{##1}}%
 \begin{rep@theorem}}%
 {\end{rep@theorem}}}
\makeatother
\newtheorem{theorem}{Theorem}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{fact}[theorem]{Fact}
\newtheoremstyle{named}{}{}{\itshape}{}{\bfseries}{.}{.5em}{\thmnote{#3}}
\theoremstyle{named}
\newtheorem*{namedtheorem}{Theorem}
%\newreptheorem{lemma}{Lemma}

\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\newcommand\mycommfont[1]{\footnotesize\ttfamily\textcolor{blue}{#1}}
\SetCommentSty{mycommfont}

\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
%% Some suggested packages, as needed:
\usepackage{natbib} % has a nice set of citation styles and commands
    \bibliographystyle{ACM-Reference-Format}
    \renewcommand{\bibsection}{\subsubsection*{References}}
\usepackage{mathtools} % amsmath with fixes and additions
% \usepackage{siunitx} % for proper typesetting of numbers and units
\usepackage{tikz} % nice language for creating drawings and diagrams

\DeclareSymbolFont{extraup}{U}{zavm}{m}{n}
\DeclareMathSymbol{\varheart}{\mathalpha}{extraup}{86}
\DeclareMathSymbol{\vardiamond}{\mathalpha}{extraup}{87}
\newcommand{\R}{\mathbb{R}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\BB}{\mathbb{B}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\OO}{{O}}
\newcommand{\oo}{{o}}
\newcommand{\ee}{\mathbf{e}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\bR}{\overline{R}}
\newcommand{\ca}{\boldsymbol{a}}
\newcommand{\xS}{\mathcal{S}}
\newcommand{\xA}{\mathbb{A}}
\newcommand{\one}{\mathbbm{1}}
\def\calA{\mathcal{A}}
\def\calB{\mathcal{B}}
\def\calD{\mathcal{D}}
\def\varV{\bm{V}}
\def\varX{\bm{X}}
\def\varXbar{\bm{\overline{X}}}
\def\varY{\bm{Y}}
\def\varZ{\bm{Z}}
\def\varW{\bm{W}}
\def\varA{\bm{A}}
\def\varAhat{\bm{\hat{A}}}
\def\varB{\bm{B}}
\def\varBhat{\bm{\hat{B}}}
\def\varx{\bm{x}}
\def\vary{\bm{y}}
\def\varz{\bm{z}}
\def\varu{\bProofm{u}}
\def\uX{\underline{X}}
\def\uY{\underline{Y}}
\def\uZ{\underline{Z}}
\def\ux{\underline{x}}
\def\uy{\underline{y}}
\def\uz{\underline{z}}
\def\e{{\varepsilon}}
\def\B{\{0,1\}}
\def\np{\mathrm{NP}}
\def\co{\mathrm{co}}
\def\eps{\varepsilon}
\def\xor{\oplus}
\def\cond{\mid}
\def\lhat{\hat{\ell}}
\providecommand\floor[1]{\lfloor#1\rfloor}
\providecommand\ceil[1]{\lceil#1\rceil}
\providecommand\blog[1]{\log_2\ceil{#1}}
\providecommand\abs[1]{\lvert#1\rvert}
\providecommand\bigabs[1]{\bigl\lvert#1\bigr\rvert}
\providecommand\ip[1]{\langle#1\rangle}
\providecommand\absip[1]{\abs{\ip{#1}}}
\DeclareMathOperator\Var{\mathrm{Var}}
\DeclareMathOperator\Cov{\mathrm{Cov}}
\DeclareMathOperator\poly{\mathrm{poly}}
\DeclareMathOperator{\pr}{\mathrm{Pr}}
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\orange}[1]{\textcolor{orange}{#1}}
\newcommand{\violet}[1]{\textcolor{violet}{#1}}
\def\p{\mathrm{P}}
\providecommand\norm[1]{\|#1\|}
\newcommand{\bracket}[1]{\left(#1\right)}
\newcommand{\sbracket}[1]{\left[#1\right]}
\makeatletter
\newcommand*{\rom}[1]{\expandafter\@slowromancap\romannumeral #1@}
\usepackage{booktabs}
